Composite likelihood inference for space-time point processes

The dynamics of a rain forest is extremely complex involving births, deaths and growth of trees with complex interactions between trees, animals, climate, and environment. We consider the patterns of recruits (new trees) and dead trees between rain forest censuses. For a current census we specify regression models for the conditional intensity of recruits and the conditional probabilities of death given the current trees and spatial covariates. We estimate regression parameters using conditional composite likelihood functions that only involve the conditional first order properties of the data. When constructing assumption lean estimators of covariance matrices of parameter estimates we only need mild assumptions of decaying conditional correlations in space while assumptions regarding correlations over time are avoided by exploiting conditional centering of composite likelihood score functions. Time series of point patterns from rain forest censuses are quite short while each point pattern covers a fairly big spatial region. To obtain asymptotic results we therefore use a central limit theorem for the fixed timespan - increasing spatial domain asymptotic setting. This also allows us to handle the challenge of using stochastic covariates constructed from past point patterns. Conveniently, it suffices to impose weak dependence assumptions on the innovations of the space-time process. We investigate the proposed methodology by simulation studies and applications to rain forest data.

==> Bib/asdasd <==
@article{jalilian:xu:waagepetersen:23,
title={A central limit theorem for a sequence of conditionally centered and $\alpha$-mixing random fields},
author={Jalilian, A. and Xu, G. and Waagepetersen, R.},
year={2022}
} 


@article{rao:09,
author={Prakasa Rao, B.L.S.},
title={Conditional independence, conditional mixing and conditional association},
journal={Annals of the Institute of Statistical Mathematics},
volume={61},
pages={441–460},
year={2009}}

@article{rasmussen:etal:07,
 ISSN = {13697412, 14679868},
 URL = {http://www.jstor.org/stable/4623291},
 abstract = {We consider statistical and computational aspects of simulation-based Bayesian inference for a spatial-temporal model based on a multivariate point process which is only observed at sparsely distributed times. The point processes are indexed by the sites of a spatial lattice, and they exhibit spatial interaction. For specificity we consider a particular dynamical spatial lattice data set which has previously been analysed by a discrete time model involving unknown normalizing constants. We discuss the advantages and disadvantages of using continuous time processes compared with discrete time processes in the setting of the present paper as well as other spatial-temporal situations.},
 author = {Jakob G. Rasmussen and Jesper Møller and Brian H. Aukema and Kenneth F. Raffa and Jun Zhu},
 journal = {Journal of the Royal Statistical Society. Series B (Statistical Methodology)},
 number = {4},
 pages = {701--713},
 publisher = {[Royal Statistical Society, Wiley]},
 title = {Continuous Time Modelling of Dynamical Spatial Lattice Data Observed at Sparsely Distributed Times},
 urldate = {2022-06-02},
 volume = {69},
 year = {2007}
}


@article{condit2017demographic,
  title={Demographic trends and climate over 35 years in the Barro Colorado 50 ha plot},
  author={Condit, Richard and P{\'e}rez, Rolando and Lao, Suzanne and Aguilar, Salom{\'o}n and Hubbell, Stephen P},
  journal={Forest Ecosystems},
  volume={4},
  number={1},
  pages={17},
  year={2017},
  publisher={SpringerOpen}
}

@article{busing1991spatial,
  title={A spatial model of forest dynamics},
  author={Busing, RT},
  journal={Vegetatio},
  volume={92},
  number={2},
  pages={167--179},
  year={1991},
  publisher={Springer}
}

@article{jacquemyn2010spatio,
  title={Spatio-temporal analysis of seedling recruitment, mortality and persistence into later life stages in the rare Primula vulgaris},
  author={Jacquemyn, H and Endels, P and Honnay, O and Wiegand, T},
  journal={Journal of Applied Ecology},
  volume={47},
  pages={431--440},
  year={2010}
}

@article{shen2013forest,
  title={Forest dynamics of a subtropical monsoon forest in Dinghushan, China: recruitment, mortality and the pace of community change},
  author={Shen, Yong and Santiago, Louis S and Ma, Lei and Lin, Guo-Jun and Lian, Ju-Yu and Cao, Hong-Lin and Ye, Wan-Hui},
  journal={Journal of Tropical Ecology},
  volume={29},
  number={2},
  pages={131--145},
  year={2013},
  publisher={Cambridge University Press}
}

@article{wiegand2009recruitment,
  title={Recruitment in tropical tree species: revealing complex spatial patterns},
  author={Wiegand, Thorsten and Mart{\'\i}nez, Isabel and Huth, Andreas},
  journal={The American Naturalist},
  volume={174},
  number={4},
  pages={E106--E140},
  year={2009},
  publisher={The University of Chicago Press}
}

@article{swaine1987dynamics,
  title={The dynamics of tree populations in tropical forest: a review},
  author={Swaine, MD and Lieberman, Diana and Putz, Francis E},
  journal={Journal of tropical ecology},
  volume={3},
  number={4},
  pages={359--366},
  year={1987},
  publisher={Cambridge University Press}
}

@article{kohyama2015demographic,
  title={Demographic properties shape tree size distribution in a Malaysian rain forest},
  author={Kohyama, Takashi S and Potts, Matthew D and Kohyama, Tetsuo I and Kassim, Abd Rahman and Ashton, Peter S},
  journal={The American Naturalist},
  volume={185},
  number={3},
  pages={367--379},
  year={2015},
  publisher={University of Chicago Press Chicago, IL}
}

@article{freville2004spatial,
  title={Spatial and temporal demographic variability in the endemic plant species Centaurea corymbosa (Asteraceae)},
  author={Fr{\'e}ville, H{\'e}l{\`e}ne and Colas, Bruno and Riba, Miquel and Caswell, Hal and Mignot, Agn{\`e}s and Imbert, Eric and Olivieri, Isabelle},
  journal={Ecology},
  volume={85},
  number={3},
  pages={694--703},
  year={2004},
  publisher={Wiley Online Library}
}

@article{rees2009integral,
  title={Integral projection models for populations in temporally varying environments},
  author={Rees, Mark and Ellner, Stephen P},
  journal={Ecological Monographs},
  volume={79},
  number={4},
  pages={575--594},
  year={2009},
  publisher={Wiley Online Library}
}

@book{lutscher2019integrodifference,
  title={Integrodifference equations in spatial ecology},
  author={Lutscher, Frithjof},
  year={2019},
  publisher={Springer}
}


@article{rathbun:cressie:94,
author = { Stephen L.   Rathbun  and  Noel   Cressie },
title = {A Space-Time Survival Point Process for a Longleaf Pine Forest in Southern Georgia},
journal = {Journal of the American Statistical Association},
volume = {89},
number = {428},
pages = {1164-1174},
year  = {1994}
}

@article{may:huth:wiegand:15,
author = {May, Felix  and Huth, Andreas  and Wiegand, Thorsten },
title = {Moving beyond abundance distributions: neutral theory and spatial patterns in a tropical forest},
journal = {Proceedings of the Royal Society B: Biological Sciences},
volume = {282},
number = {1802},
pages = {20141657},
year = {2015}
}


@article{baddeley2014logistic,
  title={Logistic regression for spatial Gibbs point processes},
  author={Baddeley, Adrian and Coeurjolly, Jean-Fran{\c{c}}ois and Rubak, Ege and Waagepetersen, Rasmus},
  journal={Biometrika},
  volume={101},
  number={2},
  pages={377--392},
  year={2014},
  publisher={Oxford University Press}
}

@article{reis:etal:13,
author = {Reis, Edna A and Gamerman, Dani and Paez, Marina S and Martins, Thiago G},
doi = {10.1016/j.csda.2012.11.008},
issn = {0167-9473},
journal = {Computational Statistics and Data Analysis},
mendeley-groups = {SPP},
pages = {146--156},
publisher = {Elsevier},
title = {{Bayesian dynamic models for space – time point processes}},
url = {http://dx.doi.org/10.1016/j.csda.2012.11.008},
volume = {60},
year = {2013}
}


@article{bezborodov:15,
  title={Markov birth-and-death dynamics of populations},
  author={Bezborodov, Viktor},
  journal={Мiждисциплiнарнi дослiдження складних систем},
  number={5},
  pages={5--47},
  year={2015}
}

@article{burslem:garwood:thomas:01,
author = {Burslem, David F R P and Garwood, Nancy C and Thomas, Sean C},
doi = {DOI: 10.1126/science.1055873},
journal = {Science (Washington D C)},
number = {5504},
pages = {607},
pmid = {1030},
title = {{Tropical forest diversity: The plot thickens}},
url = {http://www.sciencemag.org/content/291/5504/606.short},
volume = {291},
year = {2001}
}
@article{mousavi2015declustered,
author = {Mousavi-Bafrouei, Seyed Hasan and Mirzaei, Noorbakhsh and Shabani, Elham},
journal = {Annals of Geophysics},
number = {6},
title = {{A declustered earthquake catalog for the Iranian Plateau}},
volume = {57},
year = {2015}
}
@article{liang:zeger:86,
author = {Liang, K and Zeger, S L},
journal = {Biometrika},
pages = {13--22},
title = {{Longitudinal data analysis using generalized linear models}},
volume = {73},
year = {1986}
}
@article{picard:nicolas:barhen:09,
author = {Picard, Nicolas and Bar-Hen, Avner and Mortier, Fr{\'{e}}d{\'{e}}ric and Chad{\oe}uf, Jo{\"{e}}l},
journal = {Journal of Ecology},
number = {1},
pages = {97--108},
publisher = {Wiley Online Library},
title = {{Understanding the dynamics of an undisturbed tropical rain forest from the spatial pattern of trees}},
volume = {97},
year = {2009}
}
@article{wright:02,
author = {Wright, Joseph S},
journal = {Oecologia},
number = {1},
pages = {1--14},
publisher = {Springer},
title = {{Plant diversity in tropical forests: a review of mechanisms of species coexistence}},
volume = {130},
year = {2002}
}
@article{zhuang:06,
author = {Zhuang, Jiancang},
journal = {Journal of the Royal Statistical Society. Series B: Statistical Methodology},
number = {941},
pages = {634--653},
title = {{Multi-dimensional second-order residual analysis of space-time point processes and its applications in modelling earthquake data Multi-dimensional second-order residual analysis of space-time point processes and its applications in modelling earthquake da}},
volume = {68},
year = {2005}
}
@book{blangiardo:cameletti:15,
author = {Blangiardo, Marta and Cameletti, Michela},
publisher = {John Wiley {\&} Sons},
title = {{Spatial and spatio-temporal Bayesian models with R-INLA}},
year = {2015}
}
@article{Ogata1998,
author = {Ogata, Yosihiko},
doi = {10.1023/a:1003403601725},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ogata - 1998 - Space-time point-process models for earthquake occurrences.pdf:pdf},
isbn = {0020-3157},
issn = {0020-3157},
journal = {Annals of the Institute of Statistical Mathematics},
number = {2},
pages = {379--402},
title = {{Space-time point-process models for earthquake occurrences}},
url = {{\textless}Go to ISI{\textgreater}://WOS:000074666200011},
volume = {50},
year = {1998}
}
@article{Lieshout1996,
author = {Lieshout, M N M Van and Baddeley, Adrian},
doi = {10.1111/j.1467-9574.1996.tb01501.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Lieshout, Baddeley - 1996 - A non-parametric measure of spatial interaction in point patterns.pdf:pdf},
isbn = {0001-8678},
issn = {0039-0402},
journal = {Statistica Neerlandica},
keywords = {QA Mathematics},
number = {3},
pages = {344--361},
title = {{A non-parametric measure of spatial interaction in point patterns}},
url = {http://wrap.warwick.ac.uk/18756/},
volume = {50},
year = {1996}
}
@article{heinrich:klein:14,
author = {Heinrich, Lothar and Klein, Stella},
doi = {10.1007/s11203-014-9094-5},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Heinrich, Klein - 2014 - Central limit theorems for empirical product densities of stationary point processes.pdf:pdf},
issn = {13870874},
journal = {Statistical Inference for Stochastic Processes},
keywords = {Brillinger-mixing point processes,Empirical pair correlation function,Kernel-type product densities estimators,Large domain statistics,Reduced cumulant measures,{\{}Mathematical expression{\}}-goodness-of-fit tests},
pages = {1--18},
title = {{Central limit theorems for empirical product densities of stationary point processes}},
year = {2014}
}
@article{Ho2008,
author = {Ho, Lai Ping and Stoyan, Dietrich},
doi = {10.1016/j.spl.2007.11.013},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ho, Stoyan - 2008 - Modelling marked point patterns by intensity-marked Cox processes.pdf:pdf},
isbn = {0167-7152},
issn = {01677152},
journal = {Statistics and Probability Letters},
pages = {1194--1199},
title = {{Modelling marked point patterns by intensity-marked Cox processes}},
volume = {78},
year = {2008}
}
@article{getzin:wiegand:wiegand:He:08,
author = {Getzin, Stephan and Wiegand, Thorsten and Wiegand, Kerstin and He, Fangliang},
journal = {Journal of Ecology},
number = {4},
pages = {807--820},
publisher = {Wiley Online Library},
title = {{Heterogeneity influences spatial patterns and demographics in forest stands}},
volume = {96},
year = {2008}
}
@article{Yue2013,
author = {Yue, Yu Ryan and Loh, Ji Meng},
doi = {10.1080/10485252.2013.767337},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yue, Loh - 2013 - Bayesian nonparametric estimation of pair correlation function for inhomogeneous spatial point processes.pdf:pdf},
issn = {1048-5252},
journal = {Journal of Nonparametric Statistics},
number = {2},
pages = {463--474},
title = {{Bayesian nonparametric estimation of pair correlation function for inhomogeneous spatial point processes}},
url = {http://www.tandfonline.com/doi/abs/10.1080/10485252.2013.767337},
volume = {25},
year = {2013}
}
@article{Loh2014,
author = {Loh, J and Jang, W},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Loh, Jang - 2014 - Bandwidth selection for estimating the two-point correlation function of a spatial point pattern using AMSE.pdf:pdf},
journal = {Preprint},
keywords = {bandwidth selection,point correlation function,second-order clustering,spatial point patterns,two-},
pages = {1--14},
title = {{Bandwidth selection for estimating the two-point correlation function of a spatial point pattern using AMSE}},
year = {2014}
}
@book{harville:08,
address = {New York},
author = {Harville, Davide A},
isbn = {9780387783567},
pages = {651},
publisher = {Springer-Verlag},
title = {{Matrix Algebra From a Statistician's Perpective}},
year = {2008}
}
@article{Stoyan1993,
author = {Stoyan, Dietrich and Bertram, U. and Wendrock, H.},
doi = {10.1007/BF00775808},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stoyan, Bertram, Wendrock - 1993 - Estimation variances for estimators of product densities and pair correlation functions of planar poi.pdf:pdf},
issn = {00203157},
journal = {Annals of the Institute of Statistical Mathematics},
keywords = {Approximation,Poisson process,estimation variance,pair correlation function,product density,simulation},
number = {2},
pages = {211--221},
title = {{Estimation variances for estimators of product densities and pair correlation functions of planar point processes}},
url = {http://link.springer.com/10.1007/BF00775808},
volume = {45},
year = {1993}
}
@book{hubbell:01,
author = {Hubbell, S P},
number = {32},
publisher = {Princeton University Press},
series = {Monographs in Population Biology},
title = {{The unified neutral theory of biodiversity and biogeography}},
year = {2001}
}
@article{nathaniel:deangelis:09,
author = {{Nathaniel Holland}, J and DeAngelis, Donald L},
journal = {Ecology Letters},
number = {12},
pages = {1357--1366},
publisher = {Wiley Online Library},
title = {{Consumer-resource theory predicts dynamic transitions between outcomes of interspecific interactions}},
volume = {12},
year = {2009}
}
@incollection{moeller:waagepetersen:02,
author = {M{\o}ller, Jesper and Waagepetersen, Rasmus},
booktitle = {Spatial cluster modelling},
editor = {Lawson, Andrew B and Denison, David G T},
pages = {37--60},
publisher = {Chapman and Hall/CRC},
title = {{Statistical inference for {\{}C{\}}ox processes}},
year = {2002}
}
@article{prokesova:jensen:13,
author = {Proke{\v{s}}ov{\'{a}}, Michaela and Jensen, Eva B Vedel},
doi = {10.1007/s10463-012-0376-7},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Proke{\v{s}}ov{\'{a}}, Jensen - 2013 - Asymptotic Palm likelihood theory for stationary point processes.pdf:pdf},
issn = {00203157},
journal = {Annals of the Institute of Statistical Mathematics},
keywords = {Asymptotic normality,Cluster processes,Consistency,Log Gaussian Cox processes,Neyman-Scott processes,Palm likelihood,Spatial point process,Strong mixing},
number = {2},
pages = {387--412},
title = {{Asymptotic Palm likelihood theory for stationary point processes}},
volume = {65},
year = {2013}
}
@article{harms2001habitat,
author = {Harms, Kyle E and Condit, Richard and Hubbell, Stephen P and Foster, Robin B},
journal = {Journal of Ecology},
number = {6},
pages = {947--959},
publisher = {Wiley Online Library},
title = {{Habitat associations of trees and shrubs in a 50-ha Neotropical forest plot}},
volume = {89},
year = {2001}
}
@article{diggle:etal:07,
author = {Diggle, Peter J. and G??mez-Rubio, V. and Brown, P. E. and Chetwynd, A. G. and Gooding, S.},
doi = {10.1111/j.1541-0420.2006.00683.x},
file = {:home/aj/Downloads/20160510110940879(DaneshLink.com).pdf:pdf},
isbn = {0006-341X},
issn = {0006341X},
journal = {Biometrics},
keywords = {Case-control study,Ecology,Environmental epidemiology,Kernel smoothing,Monte Carlo test,Nonstationary spatial point process},
number = {2},
pages = {550--557},
pmid = {17688507},
title = {{Second-order analysis of inhomogeneous spatial point processes using case-control data}},
url = {http://doi.wiley.com/10.1111/j.1541-0420.2006.00683.x},
volume = {63},
year = {2007}
}
@article{Guan2007a,
author = {Guan, Yongtao and Loh, Ji Meng},
doi = {10.1198/016214507000000879},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan, Loh - 2007 - A Thinned Block Bootstrap Variance Estimation Procedure for Inhomogeneous Spatial Point Patterns.pdf:pdf},
isbn = {0162145070000},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {block bootstrap,inhomogeneous spatial point process,thinning},
number = {480},
pages = {1377--1386},
title = {{A Thinned Block Bootstrap Variance Estimation Procedure for Inhomogeneous Spatial Point Patterns}},
volume = {102},
year = {2007}
}
@article{picard:barhen:mortier:09,
author = {Picard, Nicolas and Bar-Hen, Avner and Mortier, Fr{\'{e}}d{\'{e}}ric and Chad{\oe}uf, Jo{\"{e}}l},
doi = {10.1111/j.1467-9469.2008.00612.x},
issn = {03036898},
journal = {Scandinavian Journal of Statistics},
keywords = {area-interaction process,exclusion formula,forest,inclusion,marked point,markov point process,metropolis algorithm,multivariate point process,process},
number = {1},
pages = {23--41},
publisher = {Wiley Online Library},
title = {{The Multi-scale Marked Area-interaction Point Process: A Model for the Spatial Pattern of Trees}},
url = {http://doi.wiley.com/10.1111/j.1467-9469.2008.00612.x},
volume = {36},
year = {2008}
}
@article{Efromovich2010,
author = {Efromovich, Sam},
doi = {10.1002/wics.97},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Efromovich - 2010 - Orthogonal series density estimation.pdf:pdf},
issn = {19395108},
journal = {Wiley Interdisciplinary Reviews: Computational Statistics},
number = {4},
pages = {467--476},
title = {{Orthogonal series density estimation}},
url = {http://doi.wiley.com/10.1002/wics.97},
volume = {2},
year = {2010}
}
@article{Lavancier2012,
archivePrefix = {arXiv},
arxivId = {1205.4818},
author = {Lavancier, Fr{\'{e}}d{\'{e}}ric and M{\o}ller, Jesper and Rubak, Ege},
eprint = {1205.4818},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Lavancier, M{\o}ller, Rubak - 2014 - Determinantal point process models and statistical inference Extended version.pdf:pdf},
journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology},
keywords = {maximum likelihood based inference,point process density,prod-,repulsiveness,simulation,spectral approach,uct densities},
pages = {1--61},
title = {{Determinantal point process models and statistical inference : Extended version}},
url = {http://arxiv.org/abs/1205.4818},
year = {2014}
}
@article{Diggle2010,
author = {Diggle, Peter J. and Menezes, Raquel and li Su, Ting},
doi = {10.1111/j.1467-9876.2009.00701.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Diggle, Menezes, Su - 2010 - Geostatistical inference under preferential sampling.pdf:pdf},
isbn = {0035-9254},
issn = {00359254},
journal = {Journal of the Royal Statistical Society. Series C: Applied Statistics},
keywords = {Environmental monitoring,Geostatistics,Log-Gaussian Cox process,Marked point process,Monte Carlo inference,Preferential sampling},
number = {2},
pages = {191--232},
title = {{Geostatistical inference under preferential sampling}},
url = {http://onlinelibrary.wiley.com/doi/10.1111/j.1467-9876.2009.00701.x/abstract$\backslash$nhttp://onlinelibrary.wiley.com/store/10.1111/j.1467-9876.2009.00701.x/asset/j.1467-9876.2009.00701.x.pdf?v=1{\&}t=gxysqm8b{\&}s=348bd334b1e8400ab4769120d4b662e650ca893b},
volume = {59},
year = {2010}
}
@article{blangiardo2013spatial,
author = {Blangiardo, Marta and Cameletti, Michela and Baio, Gianluca and Rue, H{\aa}vard},
journal = {Spatial and spatio-temporal epidemiology},
pages = {39--55},
publisher = {Elsevier},
title = {{Spatial and spatio-temporal models with R-INLA}},
volume = {7},
year = {2013}
}
@article{Hahn2012,
author = {Hahn, Ute},
doi = {10.1080/01621459.2012.688463},
file = {:home/aj/Downloads/art-345o34-2345345.pdf:pdf},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {k-function,nonparametric test,quadrat,spatial point process,subsampling},
number = {498},
pages = {754--764},
title = {{A Studentized Permutation Test for the Comparison of Spatial Point Patterns}},
url = {http://dx.doi.org/10.1080/01621459.2012.688463},
volume = {107},
year = {2012}
}
@article{zhuang:2011,
author = {Zhuang, Jiancang},
journal = {Earth, planets and space},
number = {3},
pages = {207--216},
publisher = {Springer},
title = {{Next-day earthquake forecasts for the Japan region generated by the ETAS model}},
volume = {63},
year = {2011}
}
@article{Guan2008b,
author = {Guan, Yongtao and Waagepetersen, Rasmus and Beale, Colin M},
doi = {10.1198/016214508000000391},
file = {:home/aj/Downloads/20160510105118876(DaneshLink.com).pdf:pdf},
isbn = {0162-1459},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {conditional likelihood,inhomogeneous spatial point process,pair correlation function,proportional intensity functions,residual diagnostics},
number = {482},
pages = {769--777},
title = {{Second-Order Analysis of Inhomogeneous Spatial Point Processes With Proportional Intensity Functions}},
volume = {103},
year = {2008}
}
@incollection{jensen:85,
address = {New York},
author = {Jensen, D R},
chapter = {Multivaria},
editor = {Kotz, S and Johnson, N L and Read, C B},
pages = {43--55},
publisher = {Wiley},
title = {{Encyclopedia of Statistical Sciences}},
year = {1985}
}
@book{Silverman1986,
author = {Silverman, B. W.},
booktitle = {ChapMan {\&} HALL/CRC},
doi = {10.2307/2347507},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Silverman - 1986 - Density Estimation for Statistics and Data Analysis.pdf:pdf},
isbn = {0-412-24620-1},
issn = {00359254},
keywords = {bandwidth,kde,kernel density estimation,spatial statistics,statistics},
number = {1},
pages = {120},
title = {{Density Estimation for Statistics and Data Analysis}},
url = {http://www.jstor.org/stable/10.2307/2347507?origin=crossref},
volume = {37},
year = {1986}
}
@book{diggle:03,
address = {London},
author = {Diggle, Peter J.},
isbn = {9780340740705},
pages = {159},
publisher = {Arnold},
title = {{Statistical Analysis of Spatial Point Patterns}},
year = {2003}
}
@article{gaspari:cohn:99,
author = {Gaspari, G and Cohn, S E},
journal = {Quarterly Journal of the Royal Meteorological Society},
pages = {723--757},
title = {{Construction of Correlation Functions in Two and Three Dimensions}},
volume = {125},
year = {1999}
}
@article{illian:moeller:waagepetersen:09,
author = {Illian, Janine B and M{\o}ller, Jesper and Waagepetersen, Rasmus P},
journal = {Environmental and Ecological Statistics},
number = {3},
pages = {389--405},
publisher = {Springer},
title = {{Hierarchical spatial point process analysis for a plant community with high biodiversity}},
volume = {16},
year = {2009}
}
@article{ogata:88,
author = {Ogata, Yosihiko},
journal = {Journal of the American Statistical Association},
number = {401},
pages = {9--27},
publisher = {Taylor {\&} Francis Group},
title = {{Statistical models for earthquake occurrences and residual analysis for point processes}},
volume = {83},
year = {1988}
}
@article{marzocchi:zhuang:11,
author = {Marzocchi, W and Zhuang, J},
doi = {L09310\r10.1029/2011gl047165},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Marzocchi, Zhuang - 2011 - Statistics between mainshocks and foreshocks in Italy and Southern California.pdf:pdf},
isbn = {0094-8276},
issn = {00948276},
journal = {Geophysical Research Letters},
keywords = {AFTERSHOCKS,DRIVEN,EARTHQUAKE OCCURRENCES,PREDICTION,PROBABILITIES,RATES,SEISMICITY,SHORT-TERM},
number = {9},
pages = {6},
publisher = {Wiley Online Library},
title = {{Statistics between mainshocks and foreshocks in Italy and Southern California}},
url = {{\textless}Go to ISI{\textgreater}://WOS:000290623400004},
volume = {38},
year = {2011}
}
@article{Guan2004,
author = {Guan, Yongtao and Sherman, Michael and Calvin, James a},
doi = {10.1198/016214504000001150},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan, Sherman, Calvin - 2004 - A Nonparametric Test for Spatial Isotropy Using Subsampling.pdf:pdf},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {anisotropy,isotropy,spatial statistics,subsampling,variogram},
number = {467},
pages = {810--821},
title = {{A Nonparametric Test for Spatial Isotropy Using Subsampling}},
volume = {99},
year = {2004}
}
@article{baddeley:moeller:waagepetersen:00,
archivePrefix = {arXiv},
arxivId = {math/9910011},
author = {Baddeley, Adrian and M{\o}ller, Jesper and Waagepetersen, Rasmus},
doi = {http://dx.doi.org/10.1111/1467-9574.00144},
eprint = {9910011},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baddeley, M{\o}ller, Waagepetersen - 2000 - Non- and semi-parametric estimation of interaction in inhomogeneous point patterns.pdf:pdf},
isbn = {1467-9574},
issn = {0039-0402},
journal = {Statistica Neerlandica},
keywords = {and phrases,ence,kernel estimation,markov chain monte carlo,markov point process,second-order methods,semi-parametric infer-,spatial statistics,summary statistics,thinning},
number = {3},
pages = {329--350},
pmid = {512},
primaryClass = {math},
title = {{Non- and semi-parametric estimation of interaction in inhomogeneous point patterns}},
url = {http://arxiv.org/abs/math/9910011},
volume = {54},
year = {2000}
}
@article{lombardi:marzocchi:10,
author = {Lombardi, A M and Marzocchi, Warner},
doi = {10.4401/ag-4848},
issn = {2037-416X},
journal = {Annals of Geophysics},
number = {3},
pages = {155--164},
title = {{The ETAS model for daily forecasting of Italian seismicity in the CSEP experiment}},
url = {http://www.earth-prints.org/handle/2122/6419},
volume = {53},
year = {2010}
}
@book{conway:guy:12,
author = {Conway, John H and Guy, Richard},
publisher = {Springer Science {\&} Business Media},
title = {{The book of numbers}},
year = {2012}
}
@article{Christensen2002,
author = {Christensen, Ole F and Waagepetersen, Rasmus},
doi = {10.1111/j.0006-341X.2002.00280.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Christensen, Waagepetersen - 2002 - Bayesian prediction of spatial count data using generalized linear mixed models.pdf:pdf},
issn = {0006-341X},
journal = {Biometrics},
keywords = {bayesian inference,generalized linear mixed model,geostatistics,informative prior,lange-,markov chain monte carlo,prediction,vin-hastings update,weed intensity},
number = {2},
pages = {280--286},
pmid = {12071400},
title = {{Bayesian prediction of spatial count data using generalized linear mixed models.}},
volume = {58},
year = {2002}
}
@article{vio2007ly,
author = {Vio, R and D'Odorico, V and Stoyan, H and Stoyan, D},
issn = {1432-0746},
journal = {Astronomy and Astrophysics Supplement},
keywords = {cosmology: large-scale structure of Universe,methods: data analysis,methods: statistical,quasars: absorption lines},
number = {1},
pages = {403},
publisher = {EDP Sciences},
title = {{Ly-$\alpha$ forest: efficient unbiased estimation of second-order properties with missing data}},
url = {http://adsabs.harvard.edu/cgi-bin/nph-data{\_}query?bibcode=2007A{\%}2526A...466..403V{\&}link{\_}type=ABSTRACT$\backslash$npapers://e92a9806-85b3-4e34-9639-1fb0ef0163c2/Paper/p179},
volume = {466},
year = {2007}
}
@article{comas:mateu:07,
author = {Comas, Carlos and Mateu, Jorge},
doi = {10.1002/bimj.200510268},
isbn = {0323-3847},
issn = {03233847},
journal = {Biometrical Journal},
keywords = {Correlation functions,Forest dynamics,Forest modelling,Marks,Point processes,Ripley's K,Second-order characteristics},
number = {2},
pages = {176--196},
pmid = {17476943},
publisher = {Wiley Online Library},
title = {{Modelling forest dynamics: A perspective from point process methods}},
volume = {49},
year = {2007}
}
@article{coeurjolly:meoller:14,
archivePrefix = {arXiv},
arxivId = {arXiv:1407.0249v1},
author = {Coeurjolly, Jean-fran{\c{c}}ois and M{\o}ller, Jesper},
doi = {10.3150/13-BEJ516},
eprint = {arXiv:1407.0249v1},
file = {:home/aj/Downloads/euclid.bj.1402488935.pdf:pdf},
issn = {1350-7265},
journal = {Bernoulli},
keywords = {asymptotic normality,composite likelihood,estimating equation,inhomogeneous spatial point process,strong consistency,variational estimator},
number = {3},
pages = {1097--1125},
title = {{Variational approach for spatial point process intensity estimation}},
volume = {20},
year = {2014}
}
@article{wedderburn:76,
author = {Wedderburn, R.},
journal = {Biometrika},
number = {3},
pages = {439--447},
title = {{Quasi-likelihood, generalized linear models , and the Gauss-Newton method}},
volume = {61},
year = {1974}
}
@article{baddeley:turner:05,
annote = {From Duplicate 2 (spatstat: An R Package for Analyzing Spatial Point Patterns - Baddeley, Adrian; Turner, Rolf)

URL:{\{}$\backslash$tt www.jstatsoft.org{\}}, ISSN: 1548-7660},
author = {Baddeley, Adrian and Turner, Rolf},
doi = {10.1.1.126.8464},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baddeley, Turner - 2005 - spatstat An R Package for Analyzing Spatial Point Patterns.pdf:pdf},
isbn = {9780387759685},
issn = {15487660},
journal = {Journal Of Statistical Software},
number = {6},
pages = {1--42},
pmid = {3023},
publisher = {Citeseer},
title = {{spatstat: An R Package for Analyzing Spatial Point Patterns}},
url = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.126.8464},
volume = {12},
year = {2005}
}
@book{meyn:tweedie:09,
address = {New York, NY, USA},
author = {Meyn, Sean and Tweedie, Richard L.},
doi = {10.1017/CBO9780511626630},
edition = {2nd},
isbn = {0521731828},
issn = {01621459},
pages = {594},
publisher = {Cambridge University Press},
title = {{Markov Chains and Stochastic Stability}},
url = {http://books.google.com/books?hl=en{\&}lr={\&}id=Md7RnYEPkJwC{\&}pgis=1},
year = {2009}
}
@article{Schladitz:baddeley:00,
author = {Schladitz, K and Baddeley, Adrian},
doi = {Doi 10.1111/1467-9469.00214},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Schladitz, Baddeley - 2000 - A Third Order Point Process Characteristic.pdf:pdf},
isbn = {0303-6898},
issn = {0303-6898},
journal = {Scandinavian Journal of Statistics},
keywords = {clustering,edge correction,measure,stationary point process,third factorial moment,third reduced moment measure},
number = {4},
pages = {657--671},
title = {{A Third Order Point Process Characteristic}},
url = {http://www.blackwell-synergy.com/links/doi/10.1111/1467-9469.00214/abs},
volume = {27},
year = {2000}
}
@article{Guan2008a,
author = {Guan, Yongtao},
doi = {10.1111/j.1467-9868.2007.00632.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan - 2008 - Variance estimation for statistics computed from inhomogeneous spatial point processes.pdf:pdf},
isbn = {13697412},
issn = {13697412},
journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
keywords = {Inhomogeneous spatial point process,Second-order reweighted stationarity,Thinning},
number = {1},
pages = {175--190},
title = {{Variance estimation for statistics computed from inhomogeneous spatial point processes}},
url = {http://doi.wiley.com/10.1111/j.1467-9868.2007.00632.x},
volume = {70},
year = {2008}
}
@article{ogata:katsura:91,
author = {Ogata, Yosihiko and Katsura, Koiti},
journal = {Biometrika},
number = {3},
pages = {463--474},
publisher = {Biometrika Trust},
title = {{Maximum likelihood estimates of the fractal dimension for random spatial patterns}},
volume = {78},
year = {1991}
}
@book{stein:99,
address = {New York},
author = {Stein, Michael L},
booktitle = {Journal of Statistical Planning and Inference},
doi = {10.1016/S0378-3758(00)00309-8},
isbn = {0387986294},
issn = {03783758},
number = {2},
pmid = {1764874},
publisher = {Springer Verlag},
title = {{Interpolation of spatial data: some theory for kriging.}},
volume = {96},
year = {1999}
}
@article{wood:11,
author = {Wood, Simon N.},
doi = {10.1111/j.1467-9868.2010.00749.x},
isbn = {1369-7412},
issn = {13697412},
journal = {Journal of the Royal Statistical Society. Series B: Statistical Methodology},
keywords = {Adaptive smoothing,Generalized additive mixed model,Generalized additive model,Generalized cross-validation,Marginal likelihood,Model selection,Penalized generalized linear model,Penalized regression splines,Restricted maximum likelihood,Scalar on function regression,Stable computation},
number = {1},
pages = {3--36},
title = {{Fast stable restricted maximum likelihood and marginal likelihood estimation of semiparametric generalized linear models}},
volume = {73},
year = {2011}
}
@article{rue:martino:chopin:09,
author = {Rue, H{\aa}vard and Martino, Sara and Chopin, Nicolas},
journal = {Journal of the royal statistical society: Series b (statistical methodology)},
number = {2},
pages = {319--392},
publisher = {Wiley Online Library},
title = {{Approximate Bayesian inference for latent Gaussian models by using integrated nested Laplace approximations}},
volume = {71},
year = {2009}
}
@article{ngui2014spatial,
author = {Ngui, Andr{\'{e}} Ngamini and Apparicio, Philippe and Moltchanova, Elena and Vasiliadis, Helen-Maria},
journal = {Psychiatry research},
number = {1},
pages = {20--30},
publisher = {Elsevier},
title = {{Spatial analysis of suicide mortality in Qu{\{}{\'{e}}{\}}bec: Spatial clustering and area factor correlates}},
volume = {220},
year = {2014}
}
@article{mckay:32,
author = {McKay, A T},
journal = {Biometrika},
pages = {39--44},
title = {{A Bessel function distribution}},
url = {http://www.jstor.org/stable/10.2307/2333794$\backslash$npapers3://publication/uuid/0C319FC0-E02A-4870-984F-4D6D09FA3C60},
volume = {24},
year = {1932}
}
@article{apanasovich:genton:10,
author = {Apanasovich, Tatiyana V. and Genton, Marc G.},
doi = {10.1093/biomet/asp078},
issn = {00063444},
journal = {Biometrika},
keywords = {Asymmetry,Linear model of coregionalization,Nonseparability,Positive definiteness,Space and time,Stationarity},
number = {1},
pages = {15--30},
title = {{Cross-covariance functions for multivariate random fields based on latent dimensions}},
volume = {97},
year = {2010}
}
@article{moeller:waagepetersen:07,
author = {M{\o}ller, Jesper and Waagepetersen, Rasmus},
doi = {10.1111/j.1467-9469.2007.00569.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/M{\o}ller, Waagepetersen - 2007 - Modern statistics for spatial point processes.pdf:pdf},
isbn = {3180053585},
issn = {03036898},
journal = {Scandinavian Journal of Statistics},
keywords = {Bayesian inference,Conditional intensity,Cox process,Gibbs point process,Markov chain Monte Carlo,Maximum likelihood,Perfect simulation,Poisson process,Residuals,Simulation free estimation,Summary statistics},
number = {4},
pages = {643--684},
pmid = {21953922},
publisher = {Wiley Online Library},
title = {{Modern statistics for spatial point processes}},
url = {http://www.jstor.org/stable/10.2307/4615733},
volume = {34},
year = {2007}
}
@article{Guan2011,
author = {Guan, Yongtao},
doi = {10.1111/j.1541-0420.2010.01517.x},
file = {:home/aj/Downloads/j.1541-0420.2010.01517.x.pdf:pdf},
isbn = {0006341X (ISSN)},
issn = {0006341X},
journal = {Biometrics},
keywords = {Bias correction,Spatial marked point process,Spatial point process,Subsampling},
number = {3},
pages = {926--936},
pmid = {21133879},
title = {{Bias-Corrected Variance Estimation and Hypothesis Testing for Spatial Point and Marked Point Processes Using Subsampling}},
volume = {67},
year = {2011}
}
@book{losos:leigh:04,
address = {Chicago},
editor = {Losos, E C and {Leigh Jr.}, E G},
publisher = {The University of Chicago Press},
title = {{Tropical Forest Diversity and Dynanism. Findings from a Large-Scale Plot Network}},
year = {2004}
}
@article{waagepetersen:07,
author = {Waagepetersen, Rasmus Plenge},
doi = {10.1111/j.1541-0420.2006.00667.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Waagepetersen - 2007 - An estimating function approach to inference for inhomogeneous Neyman--Scott processes.pdf:pdf},
isbn = {0006-341X},
issn = {0006341X},
journal = {Biometrics},
keywords = {Asymptotic normality,Clustering,Estimating function,Infill asymptotics,Inhomogeneous point process,Neyman-Scott point process},
number = {1},
pages = {252--258},
pmid = {17447951},
publisher = {Wiley Online Library},
title = {{An estimating function approach to inference for inhomogeneous Neyman--Scott processes}},
url = {http://doi.wiley.com/10.1111/j.1541-0420.2006.00667.x},
volume = {63},
year = {2007}
}
@article{wood:03,
author = {Wood, Simon N.},
doi = {10.1111/1467-9868.00374},
isbn = {1369-7412},
issn = {13697412},
journal = {Journal of the Royal Statistical Society. Series B: Statistical Methodology},
keywords = {Generalized additive model,Regression spline,Thin plate spline},
pages = {95--114},
title = {{Thin plate regression splines}},
volume = {65},
year = {2003}
}
@article{Stein2000,
author = {Stein, Michael L and Quashnock, Jean M and Loh, Ji Meng},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stein, Quashnock, Loh - 2000 - Estimating the K-function of a point process with an application to cosmology.pdf:pdf},
journal = {Annals of Statistics},
number = {6},
pages = {45},
title = {{Estimating the K-function of a point process with an application to cosmology}},
url = {http://arxiv.org/abs/physics/0006047},
volume = {28},
year = {2000}
}
@article{ogata:2006,
author = {Ogata, Yosihiko},
journal = {Geophysical research letters},
number = {1},
publisher = {Wiley Online Library},
title = {{Monitoring of anomaly in the aftershock sequence of the 2005 earthquake of M7. 0 off coast of the western Fukuoka, Japan, by the ETAS model}},
volume = {33},
year = {2006}
}
@article{kagan:91,
author = {Kagan, Yan Y},
journal = {Geophysical journal international},
number = {1},
pages = {135--148},
publisher = {Oxford University Press},
title = {{Likelihood analysis of earthquake catalogues}},
volume = {106},
year = {1991}
}
@article{zhang2012species,
author = {Zhang, Chunyu and Zhao, Yazhou and Zhao, Xiuhai and Gadow, K},
journal = {Silva Fenn},
title = {{Species-habitat associations in a northern temperate forest in China}},
year = {2012}
}
@book{burkhart:tome:12,
author = {Burkhart, Harold E. and Tom{\'{e}}, Margarida},
doi = {10.1007/978-90-481-3170-9},
isbn = {978-94-007-1597-4},
pages = {458},
publisher = {Springer},
title = {{Modeling Forest Trees and Stands}},
url = {http://link.springer.com/10.1007/978-90-481-3170-9},
year = {2012}
}
@article{khankeh2015model,
author = {Khankeh, Hamid Reza and Hosseini, Seyed Ali and Rezaie, Leeba and Shakeri, Jalal and Schwebel, David C},
journal = {Burns},
number = {7},
pages = {1562--1571},
publisher = {Elsevier},
title = {{A model to explain suicide by self-immolation among Iranian women: A grounded theory study}},
volume = {41},
year = {2015}
}
@article{lieshout:baddeley:99,
author = {{Van Lieshout}, M. N. M. and Baddeley, Adrian},
doi = {10.1111/1467-9469.00165},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Van Lieshout, Baddeley - 1999 - Indices of Dependence Between Types in Multivariate Point Patterns.pdf:pdf},
isbn = {0303-6898},
issn = {0303-6898},
journal = {Scandinavian Journal of Statistics},
keywords = {J-function,beta cells,bramble canes,empty space function,multi-type point pattern,myrtle disease,nearest-neighbour distance distribution function,random labelling,spatial interaction,spatial statistics},
number = {4},
pages = {511--532},
title = {{Indices of Dependence Between Types in Multivariate Point Patterns}},
url = {http://doi.wiley.com/10.1111/1467-9469.00165},
volume = {26},
year = {1999}
}
@book{condit:98,
address = {Berlin, Germany and Georgetown, Texas},
author = {Condit, Richard},
doi = {10.1007/978-3-662-03664-8},
isbn = {3540641440},
pages = {211},
publisher = {Springer-Verlag and R. G. Landes Company},
title = {{Tropical forest census plots}},
year = {1998}
}
@misc{RCoreTeam2016,
address = {Vienna, Austria},
author = {{R Core Team}},
institution = {R Foundation for Statistical Computing},
title = {{R: A Language and Environment for Statistical Computing}},
url = {https://www.r-project.org/},
year = {2016}
}
@article{Baddeley2011,
author = {Baddeley, Adrian and Rubak, Ege and M{\o}ller, Jesper},
doi = {10.1214/11-STS367},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baddeley, Rubak, M{\o}ller - 2011 - Score, Pseudo-Score and Residual Diagnostics for Spatial Point Process Models.pdf:pdf},
issn = {0883-4237},
journal = {Stat. Sci.},
keywords = {Compensator,and phrases,compensator,functional summary statistics,model,model validation,point process residuals,pseudo-likelihood},
number = {4},
pages = {613--646},
title = {{Score, Pseudo-Score and Residual Diagnostics for Spatial Point Process Models}},
url = {http://projecteuclid.org/euclid.ss/1330437942},
volume = {26},
year = {2011}
}
@article{lin:clayton:05,
author = {Lin, Pei-Sheng and Clayton, Murray K},
journal = {Annals of Statistics},
pages = {542--555},
title = {{Analysis of binary spatial data by quasi-likelihood estimating equations}},
volume = {33},
year = {2005}
}
@article{middleton2006geography,
author = {Middleton, Nicos and Sterne, Jonathan A C and Gunnell, David},
journal = {Journal of epidemiology and community health},
number = {12},
pages = {1040--1047},
publisher = {BMJ Publishing Group Ltd},
title = {{The geography of despair among 15--44-year-old men in England and Wales: putting suicide on the map}},
volume = {60},
year = {2006}
}
@article{Stoyan2000,
author = {Stoyan, Dietrich and Stoyan, Helga},
doi = {10.1111/1467-9469.00213},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stoyan, Stoyan - 2000 - Improving Ratio Estimators of Second Order Point Process Characteristics.pdf:pdf},
issn = {0303-6898},
journal = {Scandinavian Journal of Statistics},
keywords = {2nd moment measure,K function,L function,Poisson process,adapted intensity estimator,cluster process,estimator of squared intensity,hard core process,pair correlation function,pair correlation-functions,point process,ratio estimator},
number = {4},
pages = {641--656},
title = {{Improving Ratio Estimators of Second Order Point Process Characteristics}},
url = {http://doi.wiley.com/10.1111/1467-9469.00213},
volume = {27},
year = {2000}
}
@article{Ogata2006,
author = {Ogata, Yosihiko and Zhuang, Jiancang},
doi = {10.1016/j.tecto.2005.10.016},
isbn = {0040-1951},
issn = {00401951},
journal = {Tectonophysics},
keywords = {Aftershock areas,Background seismicity,ETAS model,Earthquake clusters,Modified Omori law,Space-time seismicity model,Triggering},
number = {1-2},
pages = {13--23},
title = {{Space-time ETAS models and an improved extension}},
volume = {413},
year = {2006}
}
@article{guan:shen:10,
author = {Guan, Yongtao and Shen, Ye},
doi = {10.1093/biomet/asq043},
isbn = {00063444},
issn = {00063444},
journal = {Biometrika},
keywords = {Inhomogeneous spatial point process,Intensity estimation,Poisson maximum likelihood,Weighted estimating equation},
number = {August},
pages = {867--880},
title = {{A weighted estimating equation approach for inhomogeneous spatial point processes}},
volume = {97},
year = {2010}
}
@article{baddeley:turner:00,
author = {Baddeley, Adrian and Turner, Rolf},
doi = {10.1111/1467-842X.00128},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baddeley, Turner - 2000 - Practical maximum pseudolikelihood for spatial point patterns.pdf:pdf},
isbn = {1467-842X},
issn = {1467-842X},
journal = {Australian {\&} New Zealand Journal of Statistics},
keywords = {area-interaction process,berman,dirichlet tessellation,edge effects,generalized additive models,generalized linear models,gibbs point processes,glim,hard core,inhomogeneous point process,marked point processes,markov spatial point processes,ord,pairwise interaction,process,profile pseudolikelihood,s process,soft core process,spatial clustering,turner device},
number = {3},
pages = {283--322},
pmid = {503},
title = {{Practical maximum pseudolikelihood for spatial point patterns}},
url = {http://onlinelibrary.wiley.com.proxy.lib.umich.edu/doi/10.1111/1467-842X.00128/abstract$\backslash$nhttp://onlinelibrary.wiley.com.proxy.lib.umich.edu/store/10.1111/1467-842X.00128/asset/1467-842X.00128.pdf?v=1{\&}t=hp7aamt6{\&}s=734fda260f39b2df398c153d5be84ddd9c7767e2$\backslash$n},
volume = {42},
year = {2000}
}
@article{shen2013quantifying,
author = {Shen, Guochun and He, Fangliang and Waagepetersen, Rasmus and Sun, I-Fang and Hao, Zhanqing and Chen, Zueng-Sang and Yu, Mingjian},
journal = {Ecology},
publisher = {Eco Soc America},
title = {{Quantifying effects of habitat heterogeneity and other clustering processes on spatial distributions of tree species}},
year = {2013}
}
@article{zou:hastie:tibshirani:06,
archivePrefix = {arXiv},
arxivId = {1205.0121v2},
author = {Zou, Hui and Hastie, Trevor and Tibshirani, Robert},
doi = {10.1198/106186006X113430},
eprint = {1205.0121v2},
isbn = {106186006X},
issn = {1061-8600},
journal = {Journal of Computational and Graphical Statistics},
keywords = {arrays,ca 94305,composition,d student in the,department of statistics at,edu,elastic net,email,gene expression,gene expression arrays,hui zou is a,hzou,lasso,multivariate analysis,ph,singular,singular value de-,stanford,stanford university,stat,thresholding,value decomposition},
number = {2},
pages = {2006},
pmid = {21811560},
title = {{Sparse Principal Component Analysis}},
url = {http://www.tandfonline.com/doi/abs/10.1198/106186006X113430$\backslash$nhttp://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.10.2712{\&}rep=rep1{\&}type=pdf$\backslash$nhttp://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.10.2712},
volume = {15},
year = {2004}
}
@article{gotway:stroup:97,
author = {Gotway, C A and Stroup, W W},
journal = {Journal of Agricultural, Biological, and Environmental Statistics},
pages = {157--178},
title = {{A generalized linear model approach to spatial data analysis and prediction}},
volume = {2},
year = {1997}
}
@book{Tolstov1962,
address = {New York},
author = {Tolstov, Georgi P.},
booktitle = {SpringerReference},
doi = {10.1007/SpringerReference_62084},
isbn = {0471281387},
issn = {0028-0836},
publisher = {Dover},
title = {{Fourier Series}},
url = {http://www.springerreference.com/index/doi/10.1007/SpringerReference{\_}62084},
year = {1962}
}
@article{hanisch1983reduction,
author = {Hanisch, K-H},
journal = {Statistics: A Journal of Theoretical and Applied Statistics},
number = {3},
pages = {421--435},
publisher = {Taylor {\&} Francis},
title = {{Reduction of n-th moment measures and the special case of the third moment measure of stationary and isotropic planar point processes}},
volume = {14},
year = {1983}
}
@article{politis:paparoditis:romano:98,
author = {Politis, D N and Paparoditis, E and Romano, J P},
journal = {Sankhya: The Indian Journal of Statistics},
number = {2},
pages = {274--292},
publisher = {JSTOR},
title = {{Large sample inference for irregularly space dependent opservations based on subsampling}},
volume = {60},
year = {1998}
}
@book{Baddeley2006,
author = {Baddeley, Adrian and Gregori, Pablo and Mahiques, Jorge Mateu and Stoica, Radu and Stoyan, Dietrich},
booktitle = {Case studies in spatial point process modeling},
doi = {10.1007/0-387-31144-0},
isbn = {0-387-28311-0},
pages = {323},
title = {{Case Studies in Spatial Point Process Modeling}},
url = {http://www.amazon.com/dp/0387283110},
year = {2005}
}
@book{rice:84,
author = {Rice, Elroy L},
edition = {2},
publisher = {Academic Press},
title = {{Allelopathy}},
year = {1984}
}
@article{schoenberg:2013,
author = {Schoenberg, Frederic Paik},
journal = {Bulletin of the Seismological Society of America},
number = {1},
pages = {601--605},
publisher = {Seismological Society of America},
title = {{Facilitated estimation of ETAS}},
volume = {103},
year = {2013}
}
@article{harte2014etas,
author = {Harte, D S},
journal = {Geophysical Journal International},
number = {1},
pages = {270--284},
publisher = {Oxford University Press},
title = {{An ETAS model with varying productivity rates}},
volume = {198},
year = {2014}
}
@article{wootton:emmerson:05,
author = {Wootton, J T and Emmerson, M},
journal = {Annual Review of Ecology, Evolution, and Systematics},
pages = {419--444},
title = {{Measurement of Interaction Strength in Nature}},
volume = {36},
year = {2005}
}
@article{best:ickstadt:wolpert:00,
author = {Best, Nicola G and Ickstadt, Katja and Wolpert, Robert L},
doi = {10.2307/2669744},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {air pollution,bayesian hierarchical models,continuous random fields,ecological regression,environmental,epidemiology,respiratory illness},
number = {452},
pages = {1076--1088},
title = {{Spatial Poisson Regression for Health and Exposure Data Measured at Disparate Resolutions}},
volume = {95},
year = {2000}
}
@article{illian:burslem:07,
author = {Illian, Janine and Burslem, David},
journal = {Journal de la Soci{\'{e}}t{\'{e}} Fran{\c{c}}aise de Statistiques},
keywords = {biodiversity,multivariate spatial point patterns,plant communities,spatial point processes,tropical rainforest},
pages = {9--29},
title = {{Contributions of Spatial Point Process Modelling To Biodiversity Theory}},
volume = {148},
year = {2007}
}
@article{nicolis2015windowed,
author = {Nicolis, Orietta and Chiodi, Marcello and Adelfio, Giada},
journal = {Spatial Statistics},
pages = {151--165},
publisher = {Elsevier},
title = {{Windowed ETAS models with application to the Chilean seismic catalogs}},
volume = {14},
year = {2015}
}
@article{goulard:voltz:92,
author = {Goulard, M and Voltz, M},
journal = {Mathematical Geology},
pages = {269--286},
title = {{Linear coregionalization model: Tools for estimation and choice of cross-variogram matrix}},
volume = {24},
year = {1992}
}
@article{gelfand:ghosh:clark:13,
archivePrefix = {arXiv},
arxivId = {arXiv:1312.7260v1},
author = {Gelfand, Alan E and Ghosh, Souparno and Clark, James S},
doi = {10.1214/13-STS444},
eprint = {arXiv:1312.7260v1},
issn = {0883-4237},
journal = {Statistical Science},
keywords = {Hierarchical model,Markov chain Monte Carlo,alan e,and phrases,department of statistical,duke university,durham,gelfand is professor,log Gaussian Cox process,missing data,north carolina 27708,science},
number = {4},
pages = {641--658},
pmid = {24357212},
publisher = {The Institute of Mathematical Statistics},
title = {{Scaling Integral Projection Models for Analyzing Size Demography}},
url = {http://projecteuclid.org/euclid.ss/1386078882},
volume = {28},
year = {2013}
}
@book{gaetan:guyon:10,
author = {Gaetan, Carlo and Guyon, Xavier},
booktitle = {Media},
doi = {10.1007/978-0-387-92257-7},
isbn = {9780387922560},
issn = {2191-544X},
keywords = {SPATIAL STATS,STATISTICAL,THEORY},
pages = {308},
pmid = {15928579},
publisher = {Springer},
title = {{Spatial Statistics and Modeling}},
year = {2010}
}
@article{alaghehbandan2011prospective,
author = {Alaghehbandan, Reza and Lari, Abdolaziz Rastegar and Joghataei, Mohammad-Taghi and Islami, Azar and Motavalian, Abbas},
journal = {Burns},
number = {1},
pages = {164--169},
publisher = {Elsevier},
title = {{A prospective population-based study of suicidal behavior by burns in the province of Ilam, Iran}},
volume = {37},
year = {2011}
}
@misc{hubbell:condit:foster:12,
annote = {Center for Tropical Forest Science Databases},
author = {Condit, Richard and Lao, S and P{\'{e}}rez, R and Dolins, S B and Foster, R B and Hubbell, S P},
doi = {10.5479/data.bci.20130603},
pages = {Center for Tropical Forest Science Databases},
publisher = {Center for Tropical Forest Science Databases},
title = {{Barro Colorado Forest Census Plot Data, 2012 Version}},
url = {https://repository.si.edu/handle/10088/20925},
year = {2012}
}
@article{meoller:03,
author = {M{\o}ller, Jesper},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/M{\o}ller - 2003 - Shot noise Cox processes.pdf:pdf},
journal = {Advances in Applied Probability},
number = {3},
pages = {614--640},
title = {{Shot noise Cox processes}},
url = {http://www.jstor.org/stable/1428211},
volume = {35},
year = {2003}
}
@article{nadarajah:gupta:06,
author = {Nadarajah, Saralees and Gupta, Arjun K},
journal = {Tamkang Journal of Mathematics},
pages = {185--192},
title = {{Elliptically symmetric Bessel distribution: the distribution of XY}},
volume = {37},
year = {2006}
}
@book{Chiu2013,
author = {Chiu, Sung Nok and Stoyan, Dietrich and Kendall, Wilfrid S. and Mecke, Joseph},
edition = {3},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Chiu et al. - 2013 - Stochastic Geometry and its Applications.pdf:pdf},
isbn = {9780470664810},
publisher = {Wiley},
title = {{Stochastic Geometry and its Applications}},
year = {2013}
}
@article{saman2012does,
author = {Saman, Daniel M and Walsh, Sabrina and Bor{\'{o}}wko, Anna and Others},
journal = {BMC public health},
number = {1},
pages = {1},
publisher = {BioMed Central},
title = {{Does place of residence affect risk of suicide? A spatial epidemiologic investigation in Kentucky from 1999 to 2008}},
volume = {12},
year = {2012}
}
@article{verejones1975statistical,
author = {Vere-Jones, David},
journal = {Australian Journal of Statistics},
number = {3},
pages = {134--147},
publisher = {AUSTRALIAN STATISTICAL PUBLISHING ASSOC INC C/O MR E BRINGLEY, TREASURER, GPO BOX 573, CANBERRA ACT 2601, AUSTRALIA},
title = {{STATISTICAL ASPECTS OF ESTIMATION OF EARTHQUAKE RISK}},
volume = {17},
year = {1975}
}
@article{console:jackson:kagan:2010,
author = {Console, R and Jackson, D D and Kagan, Y Y},
journal = {Pure and applied geophysics},
number = {6-7},
pages = {819--830},
publisher = {Springer},
title = {{Using the ETAS model for catalog declustering and seismic background assessment}},
volume = {167},
year = {2010}
}
@book{gerrard:69,
author = {Gerrard, Douglas James},
publisher = {Agricultural Experiment Station, Michigan State University},
title = {{Competition quotient: a new measure of the competition affecting individual forest trees}},
volume = {20},
year = {1969}
}
@article{gneiting:kleiber:schlather:11,
author = {Gneiting, Tilmann and Kleiber, William and Schlather, Martin},
doi = {10.1198/jasa.2010.tm09420},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {co-kriging,convolution,cross-correlation,gaussian spatial random field,mat{\'{e}}rn class,maximum likelihood,multi-,numerical weather prediction,positive definite,variate geostatistics},
number = {April 2014},
pages = {1167--1177},
title = {{Mat{\'{e}}rn Cross-Covariance Functions for Multivariate Random Fields}},
volume = {105},
year = {2010}
}
@article{shen:etal:09,
author = {Shen, Guochun and Yu, Mingjian and Hu, Xin-Sheng and Mi, Xiangcheng and Ren, Haibao and Sun, I Fang and Ma, Keping},
doi = {10.1890/08-1646.1},
isbn = {0012-9658},
issn = {00129658},
journal = {Ecology},
number = {11},
pages = {3033--3041},
pmid = {19967859},
title = {{Species–area relationships explained by the joint effects of dispersal limitation and habitat heterogeneity}},
url = {http://dx.doi.org/10.1890/08-1646.1},
volume = {90},
year = {2009}
}
@article{schoenberg:05,
author = {Schoenberg, Frederic Paik},
doi = {10.1016/j.jspi.2003.09.027},
issn = {03783758},
journal = {Journal of Statistical Planning and Inference},
keywords = {conditional intensity,consistency,intensity function,maximum likelihood estimation,poisson process,weighted least squares estimation},
number = {1},
pages = {79--93},
title = {{Consistent parametric estimation of the intensity of a spatial–temporal point process}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S037837580300332X},
volume = {128},
year = {2005}
}
@article{heinrich:klein:11,
author = {Heinrich, Lothar and Klein, Stella},
journal = {Statistics {\&} Risk Modeling with Applications in Finance and Insurance},
number = {4},
pages = {359--387},
title = {{Central limit theorem for the integrated squared error of the empirical second-order product density and goodness-of-fit tests for stationary point processes}},
volume = {28},
year = {2011}
}
@book{daley:verejonse:03,
address = {New York},
author = {Daley, D.J. and Vere-Jones, David},
edition = {2},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Daley, Vere-Jones - 2003 - An Introduction to the Theory of Point Processes Volume I Elementary Theory and Methods.pdf:pdf},
isbn = {0387955410},
publisher = {Springer-Verlag},
title = {{An Introduction to the Theory of Point Processes: Volume I: Elementary Theory and Methods}},
volume = {I},
year = {2003}
}
@article{Guan2006,
author = {Guan, Yongtao},
doi = {10.1111/j.1541-0420.2005.00395.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan - 2006 - Tests for Independence between Marks and Points of a Marked Point Process.pdf:pdf},
issn = {0006341X},
journal = {Biometrics},
keywords = {Mark G function,Mark K function,Marked point process,Permutation},
number = {1},
pages = {126--134},
pmid = {16542238},
title = {{Tests for Independence between Marks and Points of a Marked Point Process}},
url = {http://doi.wiley.com/10.1111/j.1541-0420.2005.00395.x},
volume = {62},
year = {2006}
}
@article{lin:et:al:11,
author = {Lin, Yi Ching and Chang, Li Wan and Yang, Kuoh Cheng and Wang, Hsiang Hua and Sun, I. Fang},
doi = {10.1007/s00442-010-1718-x},
isbn = {0029-8549},
issn = {00298549},
journal = {Oecologia},
keywords = {Dispersal limitation,Forest dynamics plots,Habitat associations,Point pattern analysis,Species coexistence},
number = {1},
pages = {175--184},
pmid = {20640861},
title = {{Point patterns of tree distribution determined by habitat heterogeneity and dispersal limitation}},
volume = {165},
year = {2011}
}
@incollection{hubbell:foster:83,
address = {Oxford},
author = {Hubbell, S P and Foster, R B},
booktitle = {Tropical Rain Forest: Ecology and Management.},
editor = {Sutton, S L and Whitmore, T C and Chadwick, A C},
pages = {25--41},
publisher = {Blackwell Scientific Publications},
title = {{Diversity of canopy trees in a Neotropical forest and implications for the conservation of tropical trees.}},
year = {1983}
}
@article{Coeurjolly2014,
archivePrefix = {arXiv},
arxivId = {1410.1448},
author = {Coeurjolly, Jean-Fran{\c{c}}ois},
doi = {10.1007/s10463-015-0536-7},
eprint = {1410.1448},
file = {:home/aj/Downloads/s10463-015-0536-7.pdf:pdf},
issn = {0020-3157},
journal = {Annals of the Institute of Statistical Mathematics},
keywords = {bahadur repre-,cox processes,robust statistics,sample quantiles},
number = {2004},
pages = {1--29},
publisher = {Springer Japan},
title = {{Median-based estimation of the intensity of a spatial point process}},
url = {http://arxiv.org/abs/1410.1448},
year = {2014}
}
@book{matern:86,
author = {Mat{\'{e}}rn, B},
publisher = {Lecture Notes in Statistics 36, Springer-Verlag, Berlin},
title = {{Spatial Variation}},
year = {1986}
}
@article{ogata:15,
author = {Ogata, Yosihiko},
journal = {Proceedings of the Institute of Statistical Mathematics},
number = {1},
pages = {105--127},
title = {{Stochastic Prediction of Earthquakes—A Strategy for the Research}},
volume = {63},
year = {2015}
}
@article{Diggle2001,
author = {Diggle, Peter J. and Brix, Anders},
doi = {10.1111/1467-9868.00315},
file = {:home/aj/Downloads/20160308230047351(DaneshLink.com).pdf:pdf},
isbn = {13697412},
issn = {1369-7412},
journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
keywords = {QA Mathematics},
number = {4},
pages = {823--841},
title = {{Spatio-temporal prediction for log-Gaussian Cox processes.}},
url = {http://www.blackwell-synergy.com/doi/abs/10.1111/1467-9868.00315},
volume = {63},
year = {2001}
}
@incollection{zhuang:ogata:verejones:06,
author = {Zhuang, Jiancang and Ogata, Yosihiko and Vere-Jones, David},
booktitle = {Case Studies in Spatial Point Process Modeling},
pages = {275--292},
publisher = {Springer},
title = {{Diagnostic analysis of space-time branching processes for earthquakes}},
year = {2006}
}
@article{zhuang:2012,
author = {Zhuang, Jiancang},
journal = {Research in Geophysics},
number = {1},
pages = {8},
title = {{Long-term earthquake forecasts based on the epidemic-type aftershock sequence (ETAS) model for short-term clustering}},
volume = {2},
year = {2012}
}
@article{Baddeley2014,
author = {Baddeley, Adrian and Diggle, Peter J. and Hardegen, Andrew and Lawrence, Thomas and Milne, Robin K. and Nair, Gopalan},
doi = {10.1890/13-2042.1},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baddeley et al. - 2014 - On tests of spatial pattern based on simulation envelopes.pdf:pdf},
isbn = {0012-9615},
issn = {15577015},
journal = {Ecological Monographs},
keywords = {Confidence bands,Conservative test,Deviation test,Global test,K function,Monte Carlo test,Null model,Pair correlation function,Pointwise test,Scale of interaction,Spatial point pattern,Variance stabilization},
number = {3},
pages = {477--489},
title = {{On tests of spatial pattern based on simulation envelopes}},
url = {http://www.esajournals.org/doi/abs/10.1890/13-2042.1},
volume = {84},
year = {2014}
}
@article{Ivanoff1982,
author = {Ivanoff, Gail},
doi = {10.1016/0304-4149(82)90040-0},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ivanoff - 1982 - Central limit theorems for point processes.pdf:pdf},
issn = {03044149},
journal = {Stochastic Processes and their Applications},
number = {2},
pages = {171--186},
title = {{Central limit theorems for point processes}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0304414982900400},
volume = {12},
year = {1982}
}
@incollection{illian:etal:06,
address = {New York},
author = {Illian, Janine and Benson, Erica and Carwford, J and Staines, H},
booktitle = {Case Studies in Spatial Point Process Modelling},
editor = {Baddeley, A and Gregori, P and Mateu, J and Stoica, R and Stoyan, D},
pages = {135--150},
publisher = {Springer},
title = {{Principal Component Analysis for Spatial Point Patterns}},
year = {2006}
}
@article{apanasovich:genton:sun:12,
author = {Apanasovich, Tatiyana V. and Genton, Marc G. and Sun, Ying},
doi = {10.1080/01621459.2011.643197},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {cokriging,correlation decay,multivariate,smoothness,spatial,valid cross-covariance},
number = {April 2014},
pages = {180--193},
publisher = {Taylor {\&} Francis},
title = {{A Valid Mat{\'{e}}rn Class of Cross-Covariance Functions for Multivariate Random Fields With Any Number of Components}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01621459.2011.643197},
volume = {107},
year = {2012}
}
@article{tanaka:13,
author = {Tanaka, Ushio},
journal = {International Journal of Applied Mathematics},
number = {4},
pages = {433--445},
publisher = {Academic Publications, Ltd.},
title = {{REMARK ON THE PALM INTENSITY OF NEYMAN-SCOTT CLUSTER POINT PROCESSES}},
volume = {26},
year = {2013}
}
@article{diggle:milne:83,
author = {Diggle, Peter J. and Milne, Robin K},
journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
keywords = {bivariate cox process,bivariate point process,bivariate spatial pattern,processes,statistical analysis of point},
number = {1},
pages = {11--21},
title = {{Bivariate Cox Processes : Some Models for Bivariate Spatial Point Patterns}},
volume = {45},
year = {1983}
}
@article{neyman:scott:58,
author = {Neyman, Jerzy and Scott, Elizabeth L},
journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
number = {1},
pages = {1--43},
publisher = {JSTOR},
title = {{Statistical Approach to Problems of Cosmology}},
url = {http://www.jstor.org/stable/2983905},
volume = {20},
year = {1958}
}
@article{Diggle2005,
author = {Diggle, Peter J. and Rowlingson, Barry and Su, Ting Li},
doi = {10.1002/env.712},
file = {:home/aj/Downloads/20160308230424666(DaneshLink.com).pdf:pdf},
issn = {11804009},
journal = {Environmetrics},
keywords = {Cox process,Disease surveillance,Gastroenteric disease,Monte Carlo inference,Spatial epidemiology,Spatio-temporal point process},
number = {5},
pages = {423--434},
title = {{Point process methodology for on-line spatio-temporal disease surveillance}},
volume = {16},
year = {2005}
}
@article{harkness:isham:83,
author = {Harkness, R D and Isham, Valerie},
journal = {Applied Statistics},
pages = {293--303},
title = {{A bivariate spatial point pattern of ants' nests}},
volume = {32},
year = {1983}
}
@article{Guan2007,
author = {Guan, Yongtao},
doi = {10.1016/j.spl.2007.04.016},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan - 2007 - A least-squares cross-validation bandwidth selection approach in pair correlation function estimations.pdf:pdf},
issn = {01677152},
journal = {Statistics {\&} Probability Letters},
keywords = {bandwidth selection,least-squares cross-validation,pair correlation function},
number = {18},
pages = {1722--1729},
publisher = {Elsevier},
title = {{A least-squares cross-validation bandwidth selection approach in pair correlation function estimations}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0167715207001575},
volume = {77},
year = {2007}
}
@article{verejons:1998,
author = {Vere-Jones, David},
journal = {Comput. Seismol},
pages = {248--263},
title = {{Probabilities and information gain for earthquake forecasting}},
volume = {30},
year = {1998}
}
@article{li:guan:14,
author = {Li, Yehua and Guan, Yongtao},
doi = {10.1080/01621459.2014.885434},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Li, Guan - 2014 - Functional Principal Component Analysis of Spatio-Temporal Point Processes with Applications in Disease Surveillance.pdf:pdf},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {composite likelihood,functional data,latent process,semiparametric methods,spatiotemporal data,splines,strong},
number = {507},
pages = {1205--1215},
pmid = {25368436},
title = {{Functional Principal Component Analysis of Spatio-Temporal Point Processes with Applications in Disease Surveillance.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/25368436},
volume = {109},
year = {2014}
}
@article{middleton2008atlas,
author = {Middleton, Nicos and Sterne, Jonathan A C and Gunnell, David J},
journal = {Health {\&} place},
number = {3},
pages = {492--506},
publisher = {Elsevier},
title = {{An atlas of suicide mortality: England and Wales, 1988--1994}},
volume = {14},
year = {2008}
}
@article{ogata:99,
author = {Ogata, Yosihiko},
doi = {10.1007/s000240050275},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ogata - 1999 - Seismicity Analysis through Point-process Modeling A Review.pdf:pdf},
isbn = {0033-4553},
issn = {0033-4553},
journal = {Pure and Applied Geophysics},
keywords = {Book: seismicity patterns...,ality of seismicity,causal relationship,etas model,modified omori formula,relative quiescence,season-,space-time models},
number = {2-4},
pages = {471--507},
publisher = {Springer},
title = {{Seismicity Analysis through Point-process Modeling: A Review}},
volume = {155},
year = {1999}
}
@incollection{illian:benson:crawford:staines:06,
author = {Illian, Janine and Benson, Erica and Crawford, John and Staines, Harry},
booktitle = {Case Studies in Spatial Point Process Modeling},
pages = {135--150},
publisher = {Springer},
title = {{Principal component analysis for spatial point processes—assessing the appropriateness of the approach in an ecological context}},
year = {2006}
}
@article{J.L.Jensen2012,
author = {{J. L. Jensen}},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/J. L. Jensen - 2012 - Asymptotic Normality of Estimates in Spatial Point Processes.pdf:pdf},
journal = {Scandinavian Journal of Statistics},
keywords = {asymptotic normality,exponential family,gibbs processes,maximum likelihood,pairwise interaction processes,pseudo likelihood,strong mixing},
number = {2},
pages = {97--109},
title = {{Asymptotic Normality of Estimates in Spatial Point Processes}},
volume = {20},
year = {2012}
}
@article{kumazawa:ogata:14,
author = {Kumazawa, Takao and Ogata, Yosihiko},
doi = {10.1214/14-AOAS759},
issn = {1941-7330},
journal = {The Annals of Applied Statistics},
keywords = {Akaike Bayesian Information Criterion,change point,induced seismic activity,time-dependent parameters,two-stage ETAS model},
number = {3},
pages = {1825--1852},
publisher = {Institute of Mathematical Statistics},
title = {{Nonstationary ETAS models for nonstandard earthquakes}},
url = {http://projecteuclid.org/euclid.aoas/1414091236},
volume = {8},
year = {2014}
}
@article{alvaro2013epidemiology,
author = {{\'{A}}lvaro-Meca, A and Kneib, T and Gil-Prieto, R and de Miguel, A Gil},
journal = {Public Health},
number = {4},
pages = {380--385},
publisher = {Elsevier},
title = {{Epidemiology of suicide in Spain, 1981--2008: a spatiotemporal analysis}},
volume = {127},
year = {2013}
}
@article{brix:moeller:01,
author = {Brix, Anders and M{\o}ller, Jesper},
doi = {10.1111/1467-9469.00249},
issn = {0303-6898},
journal = {Scandinavian Journal of Statistics},
keywords = {Metropolis adjusted Langevin algorithm,adjusted langevin algorithm,death process,inhomogeneous point patterns,log Gaussian Cox birth-death process,log gaussian cox birth,metropolis,minimum contrast estimation,pair correlation function,point patterns,predic-,prediction,third order summary statistic,time series of bivariate,time series of bivariate point patterns,tion},
number = {3},
pages = {471--488},
publisher = {Wiley Online Library},
title = {{Space-time Multi Type Log Gaussian Cox Processes with a View to Modelling Weeds}},
url = {http://onlinelibrary.wiley.com/doi/10.1111/1467-9469.00249/abstract$\backslash$nhttp://doi.wiley.com/10.1111/1467-9469.00249},
volume = {28},
year = {2001}
}
@article{moeller:soeresen:94,
author = {M{\o}ller, Jesper and S{\o}rensen, Michael},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/M{\o}ller, S{\o}rensen - 1994 - Statistical analysis of a spatial birth-and-death process model with a view to modelling linear dune fields.pdf:pdf},
issn = {0303-6898},
journal = {Scand. J. Statist.},
keywords = {control,graphical methods,likelihood methods,linear dune fields,modelling and model,nearest-neighbour birth-and-death processes on,partial likelihood,the real line},
number = {1},
pages = {1--19},
title = {{Statistical analysis of a spatial birth-and-death process model with a view to modelling linear dune fields}},
volume = {21},
year = {1994}
}
@article{ahmadi2007suicide,
author = {Ahmadi, Alireza},
journal = {Journal of burn care {\&} research},
number = {1},
pages = {30--41},
publisher = {LWW},
title = {{Suicide by self-immolation: comprehensive overview, experiences and suggestions}},
volume = {28},
year = {2007}
}
@article{Prokesova2010,
author = {Proke{\v{s}}ov{\'{a}}, Michaela},
doi = {10.5566/ias.v29.p133-141},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Proke{\v{s}}ov{\'{a}} - 2010 - Inhomogeneity in spatial cox point processes - Location dependent thinning is not the only option.pdf:pdf},
issn = {15803139},
journal = {Image Anal. Stereol.},
keywords = {Cox processes,Inhomogeneity,Moment estimation,Parameter estimation,Spatial point processes},
number = {3},
pages = {159--172},
title = {{Inhomogeneity in spatial cox point processes - Location dependent thinning is not the only option}},
volume = {29},
year = {2010}
}
@incollection{Heinrich2013,
address = {Asymptotic Methods in Statistics of Random Point Processes},
author = {Heinrich, Lothar},
booktitle = {Stochastic Geometry, Spatial Statistics and Random Fields},
doi = {10.1007/978-3-642-33305-7},
editor = {Spodarev, Evgeny},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Heinrich - 2013 - Asymptotic Methods in Statistics of Random Point Processes.pdf:pdf},
isbn = {978-3-642-33304-0},
pages = {21--48},
publisher = {Springer},
title = {{Asymptotic Methods in Statistics of Random Point Processes}},
url = {http://link.springer.com/10.1007/978-3-642-33305-7},
volume = {2068},
year = {2013}
}
@article{najafi2014assessment,
author = {Najafi, Farid and Beiki, Omid and Ahmadijouybari, Tuoraj and Amini, Saeed and Moradinazar, Mehdi and Hatemi, Masoame and Moradi, Masoud},
journal = {Journal of forensic and legal medicine},
pages = {1--5},
publisher = {Elsevier},
title = {{An assessment of suicide attempts by self-poisoning in the west of Iran}},
volume = {27},
year = {2014}
}
@book{hastie:tibshirani:90,
address = {Chichester},
author = {Wood, Simon},
publisher = {Chapman and Hall},
title = {{Generalized additive models}},
url = {http://people.bath.ac.uk/sw283/mgcv/tampere/gam.pdf},
year = {2010}
}
@article{liang:carlin:gelfand:09,
author = {Liang, S and Carlin, B P and Gelfand, A E},
journal = {The annals of applied statistics},
number = {3},
pages = {943--962},
title = {{Analysis of Minnesota colon and rectum cancer point patterns with spatial and nonspatial covariate information}},
volume = {3},
year = {2009}
}
@article{verejones:1970,
author = {Vere-Jones, David},
journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
pages = {1--62},
publisher = {JSTOR},
title = {{Stochastic models for earthquake occurrence}},
year = {1970}
}
@article{meoller:Syversveen:waagepetersen:98,
author = {M{\o}ller, Jesper and Syversveen, Anne Randi and Waagepetersen, Rasmus Plenge},
doi = {10.1111/1467-9469.00115},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/M{\o}ller, Syversveen, Waagepetersen - 1998 - Log Gaussian Cox Processes.pdf:pdf},
isbn = {03036898},
issn = {1467-9469},
journal = {Scandinavian Journal of Statistics},
keywords = {adjusted langevin algorithm,correlation function,empirical bayesian inference,ergodicity,markov chain monte carlo,metropolis-,multivariate cox processes,neyman,pair,parameter estimation,scott processes,spatial point processes,third-order properties},
number = {3},
pages = {451--482},
title = {{Log Gaussian Cox Processes}},
url = {http://onlinelibrary.wiley.com.ezp-prod1.hul.harvard.edu/doi/10.1111/1467-9469.00115/abstract$\backslash$nhttp://onlinelibrary.wiley.com.ezp-prod1.hul.harvard.edu/store/10.1111/1467-9469.00115/asset/1467-9469.00115.pdf?v=1{\&}t=hgud2cc7{\&}s=f5ec99a038a1faba2a5218a4fd3d78},
volume = {25},
year = {1998}
}
@article{Efromovich1996,
author = {Efromovich, Sam},
doi = {10.1016/0167-9473(96)00012-6},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Efromovich - 1996 - Adaptive orthogonal series density estimation for small samples.pdf:pdf},
issn = {01679473},
journal = {Computational Statistics {\&} Data Analysis},
keywords = {adaptation,density,mise,nonparametric,orthogonal series,small sample},
number = {6},
pages = {599--617},
title = {{Adaptive orthogonal series density estimation for small samples}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0167947396000126},
volume = {22},
year = {1996}
}
@article{wiegand:gunatilleke:gunatilleke:07,
author = {Wiegand, T. and Gunatilleke, S. and Gunatilleke, N.},
journal = {The American Naturalist},
number = {4},
pages = {E77--E95},
publisher = {JSTOR},
title = {{Species association in a heterogeneous Sri Lankan dipterocarp forest}},
url = {http://www.jstor.org/stable/pdfplus/10.1086/521240.pdf?acceptTC=true},
volume = {170},
year = {2007}
}
@article{Biau2015,
archivePrefix = {arXiv},
arxivId = {arXiv:1410.4029v1},
author = {Biau, G{\'{e}}rard and Cadre, Beno{\^{i}}t and Paris, Quentin and Others},
doi = {10.1007/s11203-015-9115-z},
eprint = {arXiv:1410.4029v1},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Biau et al. - 2015 - Cox process functional learning.pdf:pdf},
issn = {15729311},
journal = {Statistical Inference for Stochastic Processes},
keywords = {consistency,cox process,functional data analysis,inequality,mathematics subject classification,oracle,regularization,stochastic calculus,supervised classification},
number = {3},
pages = {in press},
publisher = {Springer Netherlands},
title = {{Cox process functional learning}},
url = {"http://dx.doi.org/10.1007/s11203-015-9115-z},
volume = {18},
year = {2015}
}
@article{barhen:picard:06,
author = {Bar-Hen, Avner and Picard, Nicolas},
doi = {10.1007/s00180-006-0008-x},
issn = {0943-4062},
journal = {Computational Statistics},
keywords = {dissimilarity,ecology,point process,simulations},
number = {3-4},
pages = {487--507},
publisher = {Physica-Verlag},
title = {{Simulation study of dissimilarity between point process}},
url = {http://link.springer.com/10.1007/s00180-006-0008-x},
volume = {21},
year = {2006}
}
@article{berman:1986,
author = {Berman, Mark},
journal = {Applied Statistics},
number = {1},
pages = {54--62},
publisher = {JSTOR},
title = {{Testing for spatial association between a point process and another stochastic process}},
volume = {35},
year = {1986}
}
@book{ripley:91,
author = {Ripley, Brian D.},
isbn = {9780521424202},
publisher = {Cambridge University Press},
title = {{Statistical Inference for Spatial Processes}},
url = {http://www.cambridge.org/gg/academic/subjects/statistics-probability/statistical-theory-and-methods/statistical-inference-spatial-processes?format=PB},
year = {1991}
}
@article{jalilian:guan:waagepetersen:12,
author = {Jalilian, Abdollah and Guan, Yongtao and Waagepetersen, Rasmus},
doi = {10.1111/j.1467-9469.2012.00795.x},
issn = {0303-6898},
journal = {Scandinavian journal of statistics, theory and applications},
keywords = {Additive random intensity,Composite likelihood,Cox process,Mat??rn covariance function,Normal variance mixture,Pair correlation function,Variance component,additive random intensity,composite likelihood,cox process,mat},
number = {1},
pages = {119--137},
pmid = {23599558},
publisher = {Wiley Online Library},
title = {{Decomposition of Variance for Spatial Cox Processes.}},
url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3626311{\&}tool=pmcentrez{\&}rendertype=abstract},
volume = {40},
year = {2013}
}
@book{karr:91,
address = {New York},
author = {Karr, A. F.},
edition = {2},
isbn = {0-8247-8532-0},
pages = {xvi+490},
publisher = {Marcel Dekker},
title = {{Point processes and their statistical inference}},
volume = {7},
year = {1991}
}
@book{lawson:13,
author = {Lawson, Andrew B},
edition = {2},
isbn = {9781466504813},
pages = {396},
publisher = {Chapman and Hall/CRC},
title = {{Bayesian disease mapping: hierarchical modeling in spatial epidemiology}},
year = {2013}
}
@book{bogachev:07,
address = {Berlin, Heidelberg},
author = {Bogachev, Vladimir I.},
doi = {10.1007/978-3-540-34514-5},
isbn = {978-3-540-34513-8},
pages = {1075},
publisher = {Springer Berlin Heidelberg},
title = {{Measure Theory}},
url = {http://link.springer.com/10.1007/978-3-540-34514-5},
year = {2007}
}
@article{groohi2006suicidal,
author = {Groohi, Bahram and {MacKay Rossignol}, Annette and {Perez Barrero}, Sergio and Alaghehbandan, Reza},
journal = {Crisis},
number = {1},
pages = {16--21},
publisher = {Hogrefe {\&} Huber Publishers},
title = {{Suicidal behavior by burns among adolescents in Kurdistan, Iran: a social tragedy}},
volume = {27},
year = {2006}
}
@article{condit:hubbell:foster:96,
author = {Condit, Richard and Hubbell, S P and Foster, R B},
journal = {Journal of Tropical Ecology},
pages = {231--256},
title = {{Changes in tree species abundance in a neotropical forest: impact of climate change}},
volume = {12},
year = {1996}
}
@article{Baddeley1997,
author = {Baddeley, Adrian and Gill, Richard D.},
doi = {10.1214/aos/1034276629},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baddeley, Gill - 1997 - Kaplan-Meier estimators of distance distributions for spatial point processes.pdf:pdf},
isbn = {0090-5364},
issn = {0090-5364, 2168-8966},
journal = {Annals of Statistics},
keywords = {Border correction method,Dilation,Distance transform,Edge corrections,Edge effects,Empty space statistic,Erosion,Functional delta-method,Influence function,K-function,Local knowledge principle,Nearest-neighbor distance,Product integration},
number = {1},
pages = {263--292},
title = {{Kaplan-Meier estimators of distance distributions for spatial point processes}},
volume = {25},
year = {1997}
}
@article{Loh2010,
author = {Loh, Ji Meng and Jang, Woncheol},
doi = {10.1111/j.1467-9876.2010.00728.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Loh, Jang - 2010 - Estimating a cosmological mass bias parameter with bootstrap bandwidth selection.pdf:pdf},
isbn = {0035-9254},
issn = {00359254},
journal = {Journal of the Royal Statistical Society. Series C: Applied Statistics},
keywords = {Adaptive bandwidth,Bandwidth selection,Bootstrap,Cosmological models,Mass bias parameter,Minimum ??2 estimation,Sloan Digital Sky Survey,Two-point correlation function},
number = {5},
pages = {761--779},
title = {{Estimating a cosmological mass bias parameter with bootstrap bandwidth selection}},
url = {{\textless}Go to ISI{\textgreater}://000283168000002},
volume = {59},
year = {2010}
}
@book{illian:penttinen:stoyan:stoyan:08,
address = {London},
author = {Illian, Janine and Penttinen, Antti and Stoyan, Helga and Stoyan, Dietrich},
booktitle = {International Statistical Review},
doi = {10.1002/9780470725160},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Illian et al. - 2008 - Statistical Analysis and Modelling of Spatial Point Patterns.pdf:pdf},
isbn = {9780470014912},
issn = {03067734},
pages = {534},
publisher = {Wiley},
title = {{Statistical Analysis and Modelling of Spatial Point Patterns}},
url = {http://doi.wiley.com/10.1111/j.1751-5823.2008.00062{\_}23.x},
volume = {76},
year = {2008}
}
@article{karacsony:06,
author = {Kar{\'{a}}csony, Zsolt},
file = {:home/aj/Downloads/7-2-karacsony.pdf:pdf},
journal = {Miskols Mathematical Notes},
keywords = {-mixing,asymptotic normality of,central limit theorem,estimators,increasing domain asymptotic,infill asymptotics,random field},
number = {2},
pages = {147--160},
title = {{A central limit theorem for mixing random fields}},
volume = {7},
year = {2006}
}
@book{D.J.2008,
author = {Daley, D.J. and Vere-Jones, David},
doi = {10.1007/b97277},
edition = {2},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Daley, Vere-Jones - 2008 - An introduction to the theory of Point Processes Volume II General Theory and Structure.pdf:pdf},
isbn = {9780387213378},
publisher = {Springer},
title = {{An introduction to the theory of Point Processes Volume II: General Theory and Structure}},
year = {2008}
}
@article{Guan2006b,
abstract = {A common assumption while analyzing spatial point processes is direction invariance, i.e., isotropy. In this article, we propose a formal nonparametric approach to test for isotropy based on the asymptotic joint normality of the sample second-order intensity function. We derive an L(2) consistent subsampling estimator for the asymptotic covariance matrix of the sample second-order intensity function and use this to construct a test statistic with a chi(2) limiting distribution. We demonstrate the efficacy of the approach through simulation studies and an application to a desert plant data set, where our approach confirms suspected directional effects in the spatial distribution of the desert plant species.},
author = {Guan, Yongtao and Sherman, Michael and Calvin, James a.},
doi = {10.1111/j.1541-0420.2005.00436.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan, Sherman, Calvin - 2006 - Assessing isotropy for spatial point processes.pdf:pdf},
isbn = {1541-0420},
issn = {0006341X},
journal = {Biometrics},
keywords = {Anisotropy,Spatial point process,Subsampling},
number = {1},
pages = {119--125},
pmid = {16542237},
title = {{Assessing isotropy for spatial point processes}},
volume = {62},
year = {2006}
}
@article{Loh2010,
author = {Loh, Ji Meng},
doi = {10.1016/j.jspi.2009.09.003},
file = {:home/aj/Downloads/1-s2.0-S0378375809002845-main.pdf:pdf},
isbn = {0378-3758},
issn = {03783758},
journal = {Journal of Statistical Planning and Inference},
keywords = {Inhomogeneous K function,Inhomogeneous point process,Marked point bootstrap,Spatial bootstrap},
number = {3},
pages = {734--749},
publisher = {Elsevier},
title = {{Bootstrapping an inhomogeneous point process}},
url = {http://dx.doi.org/10.1016/j.jspi.2009.09.003},
volume = {140},
year = {2010}
}
@article{Zhuang2002,
author = {Zhuang, Jiancang and Ogata, Yosihiko and Vere-Jones, David},
doi = {10.1198/016214502760046925},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zhuang, Ogata, Vere-Jones - 2002 - Stochastic Declustering of Space-Time Earthquake Occurrences.pdf:pdf},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {background seismicity,branching processes,earthquake declustering,space-time etas model,thinning method,variable weighted kernel estimate},
number = {458},
pages = {369--380},
title = {{Stochastic Declustering of Space-Time Earthquake Occurrences}},
volume = {97},
year = {2002}
}
@article{Stein1995,
author = {Stein, Michael L},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stein - 1995 - An approach to asymptotic inference for spatial point processes.pdf:pdf},
journal = {Statistica Sinica},
keywords = {1988,and phrases,chapters 3 and 4,correcting for edge e,e ects on,ects is a fundamental,edge e ects,interpoint distance distribution,moment function,point processes,problem in inference for,reduced second,ripley,spatial,the impact of edge,u -statistics},
pages = {221--234},
title = {{An approach to asymptotic inference for spatial point processes}},
volume = {5},
year = {1995}
}
@book{moeller:waagepetersen:04,
address = {Boca Raton},
author = {M{\o}ller, Jesper and Waagepetersen, Rasmus Plenge},
doi = {10.1201/9780203496930},
isbn = {978-0-203-49693-0},
issn = {0277-6715},
keywords = {Mathematics / Probability {\&} Statistics / Bayesian,Mathematics / Probability {\&} Statistics / General,Science / Earth Sciences / Geology},
pages = {320},
publisher = {Chapman and Hall/CRC},
title = {{Statistical Inference and Simulation for Spatial Point Processes}},
url = {https://books.google.co.uk/books?id=dBNOHvElXZ4C},
year = {2003}
}
@article{adelfio:chiodi:2015,
author = {Adelfio, Giada and Chiodi, Marcello},
journal = {Stochastic Environmental Research and Risk Assessment},
number = {2},
pages = {443--450},
publisher = {Springer},
title = {{Alternated estimation in semi-parametric space-time branching-type point processes with application to seismic catalogs}},
volume = {29},
year = {2015}
}
@book{abramowitz:stegun:65,
address = {New York},
author = {M., Abramowitz and I., Setegun and Abramowitz, M and Stegun, I},
edition = {9},
publisher = {Dover},
title = {{Handbook of Mathematical Functions}},
year = {1965}
}
@article{henrys:brown:09,
author = {Henrys, P A and Brown, P E},
journal = {Biometrics},
pages = {423--430},
title = {{Comparing clustering in two inhomogeneous spatial point processes}},
volume = {65},
year = {2009}
}
@book{guyon:91,
address = {New York},
author = {Guyon, X},
publisher = {Springer-Verlag},
title = {{Random fields on a network}},
year = {1991}
}
@article{renner:warton:13,
author = {Renner, Ian W and Warton, David I},
doi = {10.1111/j.1541-0420.2012.01824.x},
isbn = {1541-0420},
issn = {0006341X},
journal = {Biometrics},
keywords = {Habitat modeling,Location-only,Maximum entropy,Poisson likelihood,Presence-only data,Use-availability},
number = {1},
pages = {274--281},
pmid = {23379623},
publisher = {Wiley Online Library},
title = {{Equivalence of MAXENT and Poisson point process models for species distribution modeling in ecology}},
url = {http://dx.doi.org/10.1111/j.1541-0420.2012.01824.x$\backslash$nhttp://onlinelibrary.wiley.com/store/10.1111/j.1541-0420.2012.01824.x/asset/biom1824.pdf?v=1{\&}t=hwbf3gvg{\&}s=2debad2907678db75dbeaf37400f3ff0b587a212$\backslash$nhttp://onlinelibrary.wiley.com/store/10.1111/j.1541-042},
volume = {69},
year = {2013}
}
@article{stoyan:stoyan:96,
author = {Stoyan, Dietrich and Stoyan, Helga},
doi = {10.1002/bimj.4710380302},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stoyan, Stoyan - 1996 - Estimating pair correlation functions of planar cluster processes.pdf:pdf},
isbn = {0323-3847},
issn = {03233847},
journal = {Biometrical Journal},
number = {3},
pages = {259--271},
publisher = {Wiley Online Library},
title = {{Estimating pair correlation functions of planar cluster processes}},
url = {{\textless}Go to ISI{\textgreater}://WOS:A1996UM17500001},
volume = {38},
year = {1996}
}
@article{phillips2003habitat,
author = {Phillips, Oliver L and Vargas, Percy N{\'{u}}{\~{n}}ez and Monteagudo, Abel Lorenzo and Cruz, Antonio Pe{\~{n}}a and Zans, Maria-Elena Chuspe and S{\'{a}}nchez, Washington Galiano and Yli-Halla, Markku and Rose, Sam},
journal = {Journal of Ecology},
number = {5},
pages = {757--775},
publisher = {Wiley Online Library},
title = {{Habitat association among Amazonian tree species: a landscape-scale approach}},
volume = {91},
year = {2003}
}
@article{Hirukawa2015,
author = {Hirukawa, Masayuki and Sakudo, Mari},
doi = {10.1080/10485252.2014.998669},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Hirukawa, Sakudo - 2015 - Family of the generalised gamma kernels a generator of asymmetric kernels for nonnegative data.pdf:pdf},
issn = {1048-5252},
journal = {Journal of Nonparametric Statistics},
number = {1},
pages = {41--63},
title = {{Family of the generalised gamma kernels: a generator of asymmetric kernels for nonnegative data}},
url = {http://www.tandfonline.com/doi/abs/10.1080/10485252.2014.998669},
volume = {27},
year = {2015}
}
@unpublished{evans:illian:king:11,
annote = {preprint (2011), available at $\backslash$texttt{\{}http://lemur.mcs.st-andrews.ac.uk/mypapers/evaik11.pdf{\}}},
author = {Evans, Glenna and Illian, JB and King, Ruth},
booktitle = {Biometrics},
keywords = {gibbs point processes,multivariate spatial point patterns,reversible jump markov},
pages = {0--17},
title = {{Spatial Point Processes for Modelling Plant Communities in the Presence of Interaction Uncertainty}},
url = {http://lemur.mcs.st-andrews.ac.uk/mypapers/evaik11.pdf}
}
@article{schoenberg:03,
author = {Schoenberg, Frederic Paik},
doi = {10.1198/016214503000000710},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Schoenberg - 2003 - Multidimensional Residual Analysis of Point Process Models for Earthquake Occurrences.pdf:pdf},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {conditional intensity,etas model,seismology,separability,spatial,temporal marked point process},
number = {464},
pages = {789--795},
title = {{Multidimensional Residual Analysis of Point Process Models for Earthquake Occurrences}},
url = {http://www.tandfonline.com/doi/abs/10.1198/016214503000000710},
volume = {98},
year = {2003}
}
@article{hubbell:condit:foster:05,
annote = {, URL: $\backslash$texttt{\{} https://ctfs.arnarb.harvard.edu/webatlas/datasets/bci{\}}},
author = {Hubbell, Stephen P and Condit, Richard and Foster, RB},
pages = {URL https://ctfs.arnarb.harvard.edu/webatlas/datas},
title = {{Barro Colorado forest census plot data}},
year = {2005}
}
@article{helmstetter:sornette:2003,
author = {Helmstetter, Agnes and Sornette, Didier},
journal = {Geophysical research letters},
number = {11},
publisher = {Wiley Online Library},
title = {{Importance of direct and indirect triggered seismicity in the ETAS model of seismicity}},
volume = {30},
year = {2003}
}
@article{law:illian:etal:09,
author = {Law, Richard and Illian, Janine and Burslem, David F R P and Gratzer, Georg and Gunatilleke, C V S and Gunatilleke, IAUN},
journal = {Journal of Ecology},
number = {4},
pages = {616--628},
publisher = {Wiley Online Library},
title = {{Ecological information from spatial patterns of plants: insights from point process theory}},
volume = {97},
year = {2009}
}
@article{chang2011geography,
author = {Chang, Shu-Sen and Sterne, Jonathan A C and Wheeler, Benedict W and Lu, Tsung-Hsueh and Lin, Jin-Jia and Gunnell, David},
journal = {Health {\&} place},
number = {2},
pages = {641--650},
publisher = {Elsevier},
title = {{Geography of suicide in Taiwan: spatial patterning and socioeconomic correlates}},
volume = {17},
year = {2011}
}
@incollection{gelfand:banerjee:10,
address = {Boca Raton},
author = {Gelfand, AlanE and Banerjee, Sudipto},
booktitle = {Handbook of Spatial Statistics},
doi = {doi:10.1201/9781420072884-c28},
editor = {Gelfand, A E and Diggle, P J and Guttorp, P},
isbn = {978-1-4200-7287-7},
pages = {495--515},
publisher = {Chapman and Hall/CRC},
title = {{Multivariate Spatial Process Models}},
url = {http://dx.doi.org/10.1201/9781420072884-c28},
year = {2010}
}
@article{Lieshout2006,
author = {{Van Lieshout}, M. N M},
doi = {10.1007/s10463-005-0015-7},
issn = {00203157},
journal = {Annals of the Institute of Statistical Mathematics},
keywords = {Empty space function,J-function,Mark correlation function,Marked point pattern,Nearest neighbour distance distribution function,Product density,Random labelling,Reduced second moment measure,Spatial interaction,Spatial statistics},
number = {2},
pages = {235--259},
title = {{A J-function for marked point patterns}},
url = {http://link.springer.com/10.1007/s10463-005-0015-7},
volume = {58},
year = {2006}
}
@article{Rostami2016,
author = {Rostami, Mehran and Jalilian, A and Rezaei-Zangeneh, R and Salari, A},
doi = {10.5144/0256-4947.2016.7},
isbn = {0975-4466 (Electronic) 0256-4947 (Linking)},
issn = {09754466},
journal = {Ann Saudi Med},
number = {1},
pages = {7--16},
pmid = {26922682},
title = {{Factors associated with the choice of suicide method in Kermanshah Province, Iran}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/26922682},
volume = {36},
year = {2016}
}
@article{myllymaki2013deviation,
archivePrefix = {arXiv},
arxivId = {1306.1028},
author = {Myllym{\"{a}}ki, Mari and Grabarnik, Pavel and Seijo, Henri and Stoyan, Dietrich},
doi = {10.1016/j.spasta.2014.11.004},
eprint = {1306.1028},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Myllym{\"{a}}ki et al. - 2013 - Deviation test construction and power comparison for marked spatial point patterns.pdf:pdf},
issn = {22116753},
journal = {arXiv preprint arXiv:1306.1028},
keywords = {deviation test,mark-weighted k -function,marked point process,marking model,monte carlo test,multiple comparison,random labelling,simulation study},
pages = {19--34},
title = {{Deviation test construction and power comparison for marked spatial point patterns}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S2211675314000621},
volume = {11},
year = {2013}
}
@article{Kerscher2000,
archivePrefix = {arXiv},
arxivId = {astro-ph/9912088},
author = {Kerscher, Martin and Szapudi, Istv{\'{a}}n and Szalay, Alexander S.},
doi = {10.1086/312702},
eprint = {9912088},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Kerscher, Szapudi, Szalay - 2000 - A Comparison of Estimators for the Two-Point Correlation Function.pdf:pdf},
isbn = {0004-637X},
issn = {0004637X},
journal = {The Astrophysical Journal},
number = {1},
pages = {L13--L16},
primaryClass = {astro-ph},
publisher = {IOP Publishing},
title = {{A Comparison of Estimators for the Two-Point Correlation Function}},
url = {http://stacks.iop.org/1538-4357/535/i=1/a=L13},
volume = {535},
year = {2000}
}
@book{kaplan:02,
author = {Kaplan, W},
edition = {5},
isbn = {9780201799378},
publisher = {Addison-Wesley},
title = {{Advanced Calculus}},
year = {2002}
}
@article{Tanaka2014,
author = {Tanaka, Ushio and Ogata, Yosihiko},
doi = {10.1007/s10463-013-0431-z},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tanaka, Ogata - 2014 - Identification and estimation of superposed Neyman–Scott spatial cluster processes.pdf:pdf},
issn = {0020-3157},
journal = {Annals of the Institute of Statistical Mathematics},
keywords = {contact distances,likelihood functions,multi-type neyman,nearest neighbor distance function,palm intensity,processes,scott},
pages = {687--702},
title = {{Identification and estimation of superposed Neyman–Scott spatial cluster processes}},
url = {http://link.springer.com/10.1007/s10463-013-0431-z},
volume = {66},
year = {2014}
}
@article{veen:schoenberg:2008,
author = {Veen, Alejandro and Schoenberg, Frederic P},
journal = {Journal of the American Statistical Association},
number = {482},
pages = {614--624},
publisher = {Taylor {\&} Francis},
title = {{Estimation of space--time branching process models in seismology using an em--type algorithm}},
volume = {103},
year = {2008}
}
@book{stoyan:stoyan:94,
author = {Stoyan, Dietrich and Stoyan, Helga},
doi = {10.2307/2533180},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stoyan, Stoyan - 1994 - Fractals, Random Shapes and Point Fields Methods of Geometrical Statistics.pdf:pdf},
isbn = {0471937576},
issn = {0006341X},
pages = {389},
pmid = {651753},
publisher = {Wiley},
title = {{Fractals, Random Shapes and Point Fields: Methods of Geometrical Statistics}},
year = {1994}
}
@article{luo:Ming:chen:wu:ding:12,
author = {Luo, Zheng R and Ming, J Yu and Chen, De L and Wu, You G and Ding, Bing Y},
journal = {Journal of Plant Ecology},
number = {3},
pages = {346--355},
publisher = {Oxford University Press},
title = {{Spatial associations of tree species in a subtropical evergreen broad-leaved forest}},
volume = {5},
year = {2012}
}
@article{hellmund:prokesova:jensen:08,
author = {Hellmund, Gunnar and Proke{\v{s}}ov{\'{a}}, Michaela and {Vedel Jensen}, Eva B.},
doi = {10.1239/aap/1222868178},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Hellmund, Proke{\v{s}}ov{\'{a}}, Vedel Jensen - 2008 - L{\'{e}}vy-based cox point processes.pdf:pdf},
issn = {00018678},
journal = {Advances in Applied Probability},
keywords = {Cox process,Infinitely divisible distribution,Inhomogeneity,Kernel smoothing,Log Gaussian Cox process,L{\'{e}}vy basis,Mixing,Product density,Shot noise Cox process},
number = {3},
pages = {603--629},
publisher = {JSTOR},
title = {{L{\'{e}}vy-based cox point processes}},
volume = {40},
year = {2008}
}
@article{grabarnik:sarkka:09,
author = {Grabarnik, Pavel and S{\"{a}}rkk{\"{a}}, Aila},
journal = {Ecological Modelling},
number = {9},
pages = {1232--1240},
publisher = {Elsevier},
title = {{Modelling the spatial structure of forest stands by multivariate point processes with hierarchical interactions}},
volume = {220},
year = {2009}
}
@article{john2007soil,
author = {{Robert John Kyle E. Harms, Joseph B. Yavitt, Robert F. Stallard, Matthew Mirabello, Stephen P. Hubbell, Renato Valencia, Hugo Navarrete, Martha Vallejo, and Robin B. Foster}, James W Dalling and {Robert John  Kyle E. Harms, Joseph B. Yavitt, Robert F. Stallard, Matthew Mirabello, Stephen P. Hubbell, Renato Valencia, Hugo Navarrete, Martha Vallejo, and Robin B. Foster}, James W Dalling},
journal = {Pnas},
number = {3},
pages = {864--869},
publisher = {National Acad Sciences},
title = {{Soil nutrients influence spatial distributions of tropical tree species}},
url = {C:$\backslash$PDFs$\backslash$2006{\_}287.pdf C:$\backslash$PDFs$\backslash$2006{\{}{\_}{\}}287.pdf},
volume = {104},
year = {2007}
}
@article{pommerening:lemay:stoyan:11,
author = {Pommerening, Arne and LeMay, Valerie and Stoyan, Dietrich},
journal = {Ecological Modelling},
number = {3},
pages = {666--678},
publisher = {Elsevier},
title = {{Model-based analysis of the influence of ecological processes on forest point pattern formation—A case study}},
volume = {222},
year = {2011}
}
@article{Myllymaki2009,
author = {Myllym{\"{a}}ki, Mari and Penttinen, Antti},
doi = {10.1111/j.1467-9574.2009.00433.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Myllym{\"{a}}ki, Penttinen - 2009 - Conditionally heteroscedastic intensity-dependent marking of log Gaussian Cox processes.pdf:pdf},
isbn = {0039-0402},
issn = {00390402},
journal = {Statistica Neerlandica},
keywords = {Bayesian modelling,Density dependence,Marked point process,Tropical rainforest},
number = {4},
pages = {450--473},
title = {{Conditionally heteroscedastic intensity-dependent marking of log Gaussian Cox processes}},
volume = {63},
year = {2009}
}
@article{waagepetersen:guan:09,
author = {Waagepetersen, Rasmus and Guan, Yongtao},
doi = {10.1111/j.1467-9868.2008.00702.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Waagepetersen, Guan - 2009 - Two-step estimation for inhomogeneous spatial point processes.pdf:pdf},
issn = {13697412},
journal = {Journal of the Royal Statistical Society. Series B: Statistical Methodology},
keywords = {Asymptotic normality,Clustering,Estimating function,Inhomogeneous point process,Intensity function,K-function,Log-Gaussian Cox process,Minimum contrast estimation,Neyman-Scott point process},
number = {3},
pages = {685--702},
title = {{Two-step estimation for inhomogeneous spatial point processes}},
volume = {71},
year = {2009}
}
@article{Moeller2005,
author = {M{\o}ller, Jesper and Torrisi, Giovanni Luca},
doi = {10.1239/aap/1113402399},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/M{\o}ller, Torrisi - 2005 - Generalised shot noise cox processes.pdf:pdf},
issn = {00018678},
journal = {Advances in Applied Probability},
keywords = {Cluster process,Conditional simulation,Cox process,Edge effect,Generalised shot noise G Cox process,Geometric ergodicity,Markov point process,Metropolis-Hastings algorithm,Palm distribution,Perfect simulation,Shot noise Cox process,Spatial point process,Summary statistic},
number = {1},
pages = {48--74},
title = {{Generalised shot noise cox processes}},
url = {http://www.jstor.org/stable/30037315},
volume = {37},
year = {2005}
}
@article{Ogata2011,
author = {Ogata, Yosihiko},
doi = {10.5047/eps.2010.09.001},
isbn = {13438832
18805981},
issn = {1343-8832},
journal = {Earth Planets and Space},
keywords = {Anisotropic clusters,B-values,Bayesian method,Delaunay tessellation,Location dependent parameters,Probability forecasting},
number = {3},
pages = {217--229},
title = {{Significant improvements of the space-time ETAS model for forecasting of accurate baseline seismicity}},
url = {{\textless}Go to ISI{\textgreater}://WOS:000289715100007},
volume = {63},
year = {2011}
}
@book{fox1997,
author = {Fox, J},
publisher = {Sage},
title = {{Applied Regression, Linear Models, nad Related Methods}},
year = {1997}
}
@article{Hall1987,
author = {Hall, Peter},
doi = {10.1016/0047-259X(87)90001-7},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Hall - 1987 - Cross-validation and the smoothing of orthogonal series density estimators.pdf:pdf},
issn = {0047259X},
journal = {Journal of Multivariate Analysis},
number = {2},
pages = {189--206},
title = {{Cross-validation and the smoothing of orthogonal series density estimators}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0047259X87900017},
volume = {21},
year = {1987}
}
@book{chiles:delfiner:99,
author = {Chil{\`{e}}s, J. P. and Delfiner, P.},
isbn = {9781119992639},
pages = {699},
publisher = {Wiley},
series = {Probability and Statistics},
title = {{Modeling Spatial Uncertainty}},
year = {2012}
}
@article{Wu2013,
author = {Mueller, Hans-Georg and Wu, Shuang and Zhang, Zhen},
doi = {10.5705/ss.2010.162},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wu, Muller, Zhang - 2013 - Functional Data Analysis for Point Processes With Rare Events.pdf:pdf},
issn = {10170405},
journal = {Statistica Sinica},
keywords = {Bid arrival times Cox process density function fun},
pages = {1--23},
title = {{Functional data analysis for point processes with rare events}},
url = {http://www3.stat.sinica.edu.tw/statistica/j23n1/J23N11/J23N11.html},
volume = {23},
year = {2014}
}
@article{baddeley:chang:song:turner:12,
author = {Baddeley, Adrian and Chang, Y M and Y., Song and Turner, R},
doi = {10.4310/SII.2012.v5.n2.a7},
isbn = {1938-7989},
issn = {19387989},
journal = {Statistics and Its Interface},
keywords = {62G07,62H11,62M30Confidence intervals,Density e,and phrases,confidence intervals,density,estimation,ge-,gression,kernel smoothing,local likelihood,logistic re-,ological,point process intensity,poisson point process,prospectivity mapping,relative,spatial covariates},
pages = {221--236},
title = {{Nonparametric estimation of the dependence of a spatial point process on spatial covariates}},
volume = {5},
year = {2012}
}
@article{yoon2015deprivation,
author = {Yoon, Tae-Ho and Noh, Maengseok and Han, Junhee and Jung-Choi, Kyunghee and Khang, Young-Ho},
journal = {International journal of public health},
number = {8},
pages = {969--976},
publisher = {Springer},
title = {{Deprivation and suicide mortality across 424 neighborhoods in Seoul, South Korea: a Bayesian spatial analysis}},
volume = {60},
year = {2015}
}
@article{baddeley:etal:05,
author = {Baddeley, Adrian and Turner, Rolf and M{\o}ller, Jesper and Hazelton, M},
doi = {10.1111/j.1467-9868.2005.00519.x},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baddeley et al. - 2005 - Residual analysis for spatial point processes.pdf:pdf},
issn = {1369-7412},
journal = {Journal of the Royal Statistical Society: Series B (Methodological)},
keywords = {Point pattern analysis,linear regression,residual analysis},
number = {5},
pages = {617--666},
title = {{Residual analysis for spatial point processes}},
url = {http://doi.wiley.com/10.1111/j.1467-9868.2005.00519.x},
volume = {67},
year = {2005}
}
@article{harte:2012,
author = {Harte, D S},
journal = {Geophysical Journal International},
pages = {ggs026},
publisher = {Oxford University Press},
title = {{Bias in fitting the ETAS model: a case study based on New Zealand seismicity}},
year = {2012}
}
@article{diggle:zheng:durr:05,
author = {Diggle, Peter J. and Zheng, Pingping and Durr, Peter},
doi = {10.1111/j.1467-9876.2005.05373.x},
file = {:home/aj/Downloads/Diggle{\_}2005.pdf:pdf},
isbn = {1467-9876},
issn = {00359254},
journal = {Journal of the Royal Statistical Society. Series C: Applied Statistics},
keywords = {Bovine tuberculosis,Monte Carlo test,Multivariate point process,Spatial segregation},
number = {3},
pages = {645--658},
publisher = {Wiley Online Library},
title = {{Nonparametric estimation of spatial segregation in a multivariate point process: Bovine tuberculosis in Cornwall, UK}},
volume = {54},
year = {2005}
}
@article{Waagepetersen2004,
author = {Waagepetersen, Rasmus},
doi = {10.1016/j.spl.2003.10.014},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Waagepetersen - 2004 - Convergence of posteriors for discretized log Gaussian Cox processes.pdf:pdf},
issn = {01677152},
journal = {Statistics and Probability Letters},
keywords = {Bayesian inference,Discretization,Log Gaussian Cox process,Monte Carlo,Point processes,Posterior},
number = {3},
pages = {229--235},
title = {{Convergence of posteriors for discretized log Gaussian Cox processes}},
volume = {66},
year = {2004}
}
@article{hubbell:etal:99,
author = {Hubbell, S P and Foster, R B and O'Brien, S T and Harms, K E and Condit, Richard and Wechsler, B and Wright, S J and de Lao, S},
journal = {Science},
pages = {554--557},
title = {{Light gap disturbances, recruitment limitation, and tree diversity in a neotropical forest}},
volume = {283},
year = {1999}
}
@article{Drikvandi2011,
author = {Drikvandi, Reza and Modarres, Reza and Jalilian, Abdullah H.},
journal = {Computational Statistics and Data Analysis},
keywords = {Bootstrap,Ranked set sampling,Simulation,Symmetry},
number = {4},
pages = {1807--1814},
title = {{A bootstrap test for symmetry based on ranked set samples}},
volume = {55},
year = {2011}
}
@article{stoyan:penttinen:00,
author = {Stoyan, Dietrich and Penttinen, Antti},
journal = {Statistical Science},
number = {1},
pages = {61--78},
publisher = {Institute of Mathematical Statistics},
title = {{Recent applications of point process methods in forestry statistics}},
volume = {15},
year = {2000}
}
@article{Guan2006a,
author = {Guan, Yongtao},
doi = {10.1198/016214506000000500},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan - 2006 - A composite likelihood approach in fitting spatial point process models.pdf:pdf},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {composite likelihood,spatial point process},
number = {476},
pages = {1502--1512},
title = {{A composite likelihood approach in fitting spatial point process models}},
url = {http://www.tandfonline.com/doi/abs/10.1198/016214506000000500},
volume = {101},
year = {2006}
}
@article{di2015isc,
author = {{Di Giacomo}, Domenico and Harris, James and Villase{\~{n}}or, Antonio and Storchak, Dmitry A. and Engdahl, E. Robert and Lee, William H.K.},
doi = {10.1016/j.pepi.2014.06.003},
issn = {00319201},
journal = {Physics of the Earth and Planetary Interiors},
keywords = {Instrumental data},
pages = {14--24},
publisher = {Elsevier},
title = {{ISC-GEM: Global Instrumental Earthquake Catalogue (1900–2009), I. Data collection from early instrumental seismological bulletins}},
url = {http://www.sciencedirect.com/science/article/pii/S0031920114001484},
volume = {239},
year = {2015}
}
@article{Guan2008,
author = {Guan, Yongtao},
doi = {10.1198/016214508000000526},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guan - 2008 - On Consistent Nonparametric Intensity Estimation for Inhomogeneous Spatial Point Processes.pdf:pdf},
issn = {0162-1459},
journal = {Journal of the American Statistical Association},
keywords = {inhomogeneous spatial point processes,intensity estimation,kernel smoothing,sliced inverse regression},
number = {483},
pages = {1238--1247},
title = {{On Consistent Nonparametric Intensity Estimation for Inhomogeneous Spatial Point Processes}},
volume = {103},
year = {2008}
}
@article{Tanaka2008,
author = {Tanaka, Ushio and Ogata, Yosihiko and Stoyan, Dietrich},
doi = {10.1002/bimj.200610339},
file = {:home/aj/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tanaka, Ogata, Stoyan - 2008 - Parameter estimation and model selection for Neyman-Scott point processes.pdf:pdf},
issn = {03233847},
journal = {Biometrical Journal},
keywords = {AIC,Generalized thomas model,Inverse-power type model,K-function,Multi-type clusters,Pair-correlation function,Palm intensity function,Palm likelihood function,Thomas model},
pages = {43--57},
pmid = {17640081},
title = {{Parameter estimation and model selection for Neyman-Scott point processes}},
volume = {50},
year = {2008}
}
@article{bolthausen:82,
author = {Bolthausen, E},
journal = {The Annals of Probability},
number = {4},
pages = {1047--1050},
title = {{On the central limit theorem for stationary mixing random fields}},
url = {http://www.jstor.org/stable/2243560},
volume = {10},
year = {1982}
}

